Does the Order of Fine-tuning Matter and Why?

To improve the performance on a target task, researchers have fine-tuned language models with an intermediate task before the target task of interest. However, previous works have focused on the pre-trained language models and downstream tasks in Natural Language Processing (NLP) and considered only one intermediate task. The effect of fine-tuning multiple intermediate tasks and their ordering on target task performance has not been fully explored in Software Engineering. In this study, we perform the first empirical study on analyzing the impact of task ordering on target task performance. Experimental results show that there is an impact of task ordering on target task performance by up to 6% of performance gain and up to 4% of performance loss. To explain such an impact, we consider a variety of potential factors, including the characteristics of dataset (syntactic similarity and semantic similarity analysis, dataset size), model (probing task and attention analysis), and task (task affinity analysis). Our study provides Software Engineering researchers and practitioners with insights into the effect of task orderings and how to select the one that is cost-effective while achieving the best performance gain.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figures/01-intro.tex <==
%!TEX root = main.tex

\section{Introduction}
%!TEX root = main.tex
\label{sec:intro}

\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\footnotetext[1]{The ﬁrst two authors contributed equally to this work.}
\renewcommand*{\thefootnote}{\arabic{footnote}}

% background of pre-trained source code language models and their fine-tuning for SE tasks
%\hl{Very long sentence}
%Natural Language Processing (NLP) has witnessed the advancement of large pre-trained language models (e.g., BERT~\cite{devlin2018bert}, BART~\cite{lewis2019bart}, and T5~\cite{raffel2020exploring}) trained on a natural language corpus. 

%With the advancement of self-supervised learning where annotated training data can be automatically generated from text corpus in the field of Natural Language Processing (NLP), large language models started to play an important role in automating different NLP tasks (i.e. text classification, and question answering). These models are firstly pre-trained with an extensive text corpus so that its parameter weights encode general linguistic and commonsense knowledge about the language~\cite{devlin2018bert}. To apply the models to downstream tasks, they are further fine-tuned on a task-specific dataset (i.e. human-annotated training data that is usually costly to collect) in a supervised manner. The whole process can also be seen as a transfer learning approach where the linguistic knowledge learned during the pre-training stage is transferred to the fine-tuning stage of the downstream task, which usually expedites the whole training process and improves the model performance.

The recent advancements in self-supervised learning, where annotated training data can be automatically generated from text corpus have led to increasing the importance of large language models in automating various Natural Language Processing (NLP) tasks such as text classification and question answering. These models undergo pre-training on an extensive text corpus, during which their parameter weights are trained to encode general linguistic and commonsense knowledge about the language~\cite{devlin2018bert}. To apply these models to downstream tasks, they undergo further fine-tuning on a task-specific dataset, which typically involves human-annotated training data that is expensive to acquire in a supervised manner. This entire process can be considered as a transfer learning approach where the linguistic knowledge acquired during the pre-training phase is transferred through the fine-tuning phase to the downstream task, resulting in an accelerated training process and improved model performance.


% What people have done about fine-tuning an intermediate task before the target task in NLP
%To further improve model performance on downstream tasks, researchers in NLP have also examined fine-tuning with another task before the \textit{target task} of interest~\cite{phang2018sentence, wang2018glue, wang2018can, vu2020exploring, pruksachatkun2020intermediate}. This task is referred to as an \textit{intermediate task} that is supposed to accumulate additional knowledge for the downstream target task to perform even better than the pre-trained model that is directly fine-tuned on the target task dataset. However, previous NLP research~\cite{phang2018sentence} has revealed that arbitrarily selecting intermediate tasks can even negatively affect the target task's performance~\cite{wang2018glue}, which is referred to as \textit{negative transfer}. To identify the conditions for a \textit{positive transfer} (a transfer learning between intermediate task and target task that actually brings performance gains for the target task) between an intermediate task and a target task, a variety of factors have been considered, including the learned linguistic skills~\cite{pruksachatkun2020intermediate}, dataset size, and data text domain~\cite{vu2020exploring}.



To further improve model performance on downstream tasks, researchers in NLP have investigated fine-tuning with an intermediate task before the target task to enhance model performance on downstream tasks~\cite{phang2018sentence, wang2018glue, wang2018can, vu2020exploring, pruksachatkun2020intermediate}. The intermediate task is designed to accumulate additional knowledge that can help the downstream target task achieve superior performance compared to a pre-trained model that is directly fine-tuned on the target task dataset. However, previous NLP studies~\cite{phang2018sentence} have demonstrated that selecting intermediate tasks arbitrarily can result in \textit{negative transfer}, whereby the target task's performance is adversely affected~\cite{wang2018glue}. Therefore, researchers have investigated various factors, including the learned linguistic skills~\cite{pruksachatkun2020intermediate}, dataset size, and data text domain~\cite{vu2020exploring}, to identify the conditions for \textit{positive transfer}, referring to a transfer learning between the intermediate task and the target task that leads to performance gains for the target task.



%Following the success of pre-trained large language models in NLP, language models pre-trained on a large corpus of source code such as CodeBERT~\cite{feng2020codebert}, PLBART~\cite{ahmad2021unified}, and CodeT5~\cite{wang2021codet5} have demonstrated remarkable performances in a variety of code intelligence tasks, spanning from code understanding (e.g., defect detection) to code generation (e.g., code translation). \hl{Very long sentence}.

%\textcolor{blue} {In addition, researchers have also investigated the effect of training DL models on a chain of datasets from various tasks. For example, Ahmed et al. reported that programs in different languages solving the same problem tend to use similar identifiers, keywords and operators. They found that high-capacity DL models can learn interlingua: shared semantic representation between languages. Specifically, they have showed that one can enhance the models' performance on a specific SE task by training on a task-specific dataset that contains multiple different programming languages. The underlying explanation is that the shared knowledge hidden in the keywords, operators and identifiers existing in the datasets of different programming languages can boost model's performance.}

% based on existing works in NLP, we found some limitations, and the limitations motivate our work in SE

%\hl{Add a figure showing one task in between and multiple tasks and reference it from this para}
Despite these studies providing a foundational understanding of transferability between downstream tasks and the conditions for a positive transfer, they only considered a single intermediate task fine-tuned before the target task. In Figure \ref{fig:multiplefinetune}, we present the difference between single intermediate task fine-tuning and multiple intermediate task fine-tuning. We posit that fine-tuning more than one intermediate task in some specific orders may further improve the model's performance as the model may accumulate more diverse knowledge from multiple task-specific datasets. However, the influence of fine-tuning multiple intermediate tasks on the target task's performance has not been explored. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/multi-inter2.png}
    \caption{Single Intermediate Task Fine-tuning VS multiple Intermediate Task Fine-tuning}
    \label{fig:multiplefinetune}
\end{figure}

Following the success of pre-trained large language models in NLP, language models pre-trained on a large corpus of source code such as CodeBERT~\cite{feng2020codebert}, PLBART~\cite{ahmad2021unified}, and CodeT5~\cite{wang2021codet5} have demonstrated remarkable performances in a variety of code intelligence tasks, spanning from code understanding (e.g., defect detection) to code generation (e.g., code translation). As source code possesses distinct features different from natural languages, such as its inherent syntactic constraints and semantic structures~\cite{casalnuovo2019studying, niu2023empirical}, the findings from NLP may not directly apply to Software Engineering (SE) tasks that primarily involve source code. The transferability between SE tasks remains an area requiring further understanding to enhance the model's performance even more.

%\hl{Why is it important to understand? what would be the benefit of doing this. Need few lines talking about that}

To shed light on SE task transferability and how SE tasks affect each other, we ask our first research question: 

\textbf{RQ1: Does the fine-tuning task ordering with multiple intermediate SE tasks matter for target task performance?}

% overview of the experiments we did to answer RQ1, since we need to address why we only use codebert and the 4 SE tasks, we need to mention them here
To answer our RQ1, we select four SE tasks from CodeXGLUE benchmark suite~\cite{lu2021codexglue}, namely, Clone Detection (CD)~\cite{svajlenko2014towards}, Defect Detection (DD)~\cite{zhou2019devign}, Code Repair (CR)~\cite{tufano2019empirical}, and Code Translation (CT)~\cite{nguyen2015divide}. It should be noted that the selection of the four tasks is driven by the aim of exploring tasks that involve various methods of utilizing and manipulating code. Specifically, our investigation includes tasks that focus on (i) transforming code with the goal of changing its behavior (CR) and preserving its behavior (CT); (ii) understanding the code as to whether it contains a bug (DD); and (iii) understanding the code as to whether it is semantically similar to another piece of code (CD). Such a group of tasks contributes to increasing the generalizability of our findings. We should note that we experiment with four SE tasks in total to show whether their ordering matters. We believe the four tasks are representative enough to analyze the potential reasons contributing to the target task's performance difference.

As for the pre-trained model, we picked CodeBERT~\cite{feng2020codebert} since it has been widely evaluated and compared in a large number of studies~\cite{kanade2020learning,lu2021codexglue,wang2021codet5}. In order to generate task-specific outputs, we either use a randomly initialized Transformer as the decoder for code generation tasks or softmax layers for other tasks (e.g., classification tasks). In our experiments, we first fine-tune each of the four tasks directly without any intermediate tasks in between to obtain the \textit{baseline models}. Then, we conduct the fine-tuning on SE tasks sequentially to collect \textit{fine-tuning chain models}. We fine-tune all permutations of any two, three, or all four tasks in sequential chains. That is, the chains' lengths range from two to lengths of four (e.g., two, three, or four tasks trained sequentially in a fine-tuning chain) that involve any possible permutations of two, three, or four tasks. We use \textit{task ordering} to refer to a sequential fine-tuning chain of intermediate and target tasks with the pre-trained model. All the permutations of tasks are fine-tuned sequentially with the goal of discovering task ordering patterns that either always bring performance gain or loss for a target task (i.e., positive/negative transfer), which may indicate the fine-tuning task ordering does matter for the target task. To make our experiments manageable, we did not fine-tune tasks with pre-trained models other than CodeBERT, as we believe our findings on CodeBERT can be easily generalized to other language models.

%\hl{Our findings suggest that fine-tuning some tasks in a specific order does boost the performance of a target task, while fine-tuning in other orders could hurt target task's performance.IA: giving away results. Don't }




Next, we are interested in explaining why task ordering matters. This prompts us to ask our second research question:

\textbf{RQ2: Why does the fine-tuning task ordering impact the performance of the target task?}

% overview of the characteristics we consider to answer RQ2, do we need to elaborate on all of them?
To answer RQ2, we provide explanations from a variety of dimensions, including characteristics of training dataset, SE task, and model. In each dimension, we conduct experiments to investigate their associations with the impact of task orderings.

% Why we only selected codebert and why we only picked the 4 SE tasks
%We should note that we are only trying to analyze and explain the presence of general impact of different fine-tuning orders of intermediate tasks on the performance of the target task, rather than figuring out the exact chain of fine-tuning that boosts/hurts a target task's performance for a specific pre-trained language model. \hl{this is contradicting what you have setup so far. and confusing}


%Therefore, we select CodeBERT as our experimental target since it's one of the most widely-used source code language models. Similarly, we only experiment with 4 SE tasks in total to show whether order matters. We believe the 4 tasks are representative for us to analyze the potential reasons that contribute to the performance difference of the target task. \hl{said somethis similar in a previuous para, this sentence needs to moved there.}

Finally, we analyze the practical implications of our findings and ask our third research question:

\textbf{RQ3: What are the time-performance trade-offs when choosing different task orderings to fine-tune?}
To answer RQ3, we analyze the fine-tuning chain models of positive transfer and their training time to find out whether certain trade-offs between training time and performance gain exist. Then, we provide insights into selecting the most cost-effective task ordering for a given target task.

%\hl{The following two points are redundant}
To summarize, the significance of our contributions are following:

(1) We show that different task orderings could impact the target task performance differently.

(2) We analyze the possible factors in data, task, and model dimension that could help to explain why task ordering matters.

(3) We analyze the training trade-offs of task orderings to provide implications for practitioners and researchers.

%The remainder of this paper is organized as follows: In Section \ref{sec:relatedworks}, we review related research on fine-tuning language models. We outline our experimental setup in Section \ref{sec:method}. Next, we present our model evaluation results in Section \ref{sec:results} and the analyses in Section \ref{sec:discussion}. Then, we discuss the implications for our study in Section \ref{sec:impl}. Section \ref{sec:ttv} shows potential threats to the validity of our reported findings. Finally, we conclude with a summary of the key findings in Section \ref{sec:conclusion}.




==> figures/02-relatedworks.tex <==
%!TEX root = main.tex
\section{Related Works}
\label{sec:relatedworks}

\subsection{Fine-tuning of Pre-trained Language Models for SE tasks}
Traditional NLP models were built to be task-specific. They were trained on task-specific data with weights or parameters randomly initialized, where specific learning objective functions were used. However, for many learning tasks, collecting human-annotated data of high quality can be both challenging and costly. To address this challenge, researchers came up with language model \textit{pre-training}~\cite{dai2015semi, radford2018improving}. Rather than training the models from scratch with randomly initialized weights, the models are \textit{pre-trained} on large text corpora so that they learn the general knowledge about the target natural language. Then the learned knowledge can be transferred to the downstream tasks by fine-tuning the pre-trained models with a relatively small amount of task-specific data~\cite{lu2021codexglue}. This pre-training approach has proven effective in improving the models' performance compared to the traditional approach~\cite{lu2021codexglue, chen2021evaluating}.

% more about pre-trained NL model and their counterparts in SE
Pre-trained language models can be classified into autoregressive language models~\cite{brown2020language}, masked language models~\cite{devlin2018bert}, and encoder-decoder~\cite{lewis2019bart} language models based on their pre-training objectives. Autoregressive language models employ "generative pre-training," predicting the next token in a sequence (e.g., GPT-3)~\cite{brown2020language, recchia2021teaching}. Masked language models predict masked tokens using the remaining token sequence as context (e.g., BERT)~\cite{devlin2018bert}, while encoder-decoder language models are trained on sequence-to-sequence tasks, excelling in translation and summarization tasks (e.g., T5, BART)~\cite{lewis2019bart, raffel2020exploring}. Recently, pre-trained natural language models have been adapted for source code, such as CodeGPT/Codex~\cite{chen2021evaluating} (based on GPT-3~\cite{brown2020language}), CodeBERT/GraphCodeBERT~\cite{feng2020codebert, guo2020graphcodebert} (based on BERT~\cite{devlin2018bert, liu2019roberta}), and CodeT5~\cite{wang2021codet5} (based on T5~\cite{raffel2020exploring}). Those language models have been evaluated and fine-tuned for various SE tasks such as code repair, and code translation, demonstrating promising results. 

\subsection{Transfer Learning from Intermediate Task fine-tuning}
To further enhance state-of-the-art model performance on downstream NLP tasks, researchers have introduced an additional fine-tuning strategy: first fine-tuning the pre-trained model on an intermediate task before the target task of interest.~\cite{phang2018sentence, wang2018can, wang2018glue}. However, this approach does not consistently improve target task performance and may even be detrimental, depending on the chosen intermediate task.~\cite{wang2018can}. 

To investigate the condition of positive transfer and to avoid negative transfer~\cite{torrey2010transfer}, many research works have been done. Pruksachatkun et al.~\cite{pruksachatkun2020intermediate} examined the linguistic skills acquired from intermediate tasks that could potentially contribute to positive transfer on a target task. Their findings suggested that although a model might learn certain skills from an intermediate task, these skills may not necessarily benefit the target task. Change et al. ~\cite{chang2021rethinking} investigated various factors that could influence the effectiveness of intermediate task fine-tuning, including the training dataset sizes of both intermediate and target tasks. Furthermore, Vu et al.~\cite{vu2020exploring} carried out extensive experiments on 33 NLP tasks to illuminate the transferability between these tasks, discovering that the similarity between the intermediate and target tasks, as well as their training data domains, are important factors for positive transfer. 

Despite these previous studies providing valuable insights into transferability among different downstream tasks, they only focused on NLP tasks, not SE tasks, which primarily involve program source code instead of natural language, making it a non-trivial task to adapt learnings from NLP tasks to SE tasks. Consequently, there remains a gap in understanding transferability between SE tasks. Moreover, these NLP studies only considered a single intermediate task, neglecting the potential effects of multiple intermediate tasks and their fine-tuning orderings on the target task. It is worth noting that Mastropaolo et al.~\cite{mastropaolo2022using} explored the advantages of transfer learning for SE tasks, but their investigation was limited to multi-task learning with only four SE tasks (muti-task learning aims to train tasks in parallel using a shared representation, while our approach is training tasks sequentially in chains),leaving the impacts of sequential intermediate-target task fine-tuning unexplored. In this paper, we take the first steps towards exploring that.

% \subsection{UNDERSTANDING AND IMPROVING INFORMATION TRANSFER IN MULTI-TASK LEARNING}
% Multi-task learning is a approach paradigm that use a shared feature representation for all tasks. Wu et.al focus on the transfer of task information in multi-task learning. They studied the architecture with a shared module for all tasks and a separate output module for each task. They reported that the transfer rate and transfer type is strongly associated with the data alignment. In other words, data alignment determines how well the knowledge from one task to another task and whether the transfer is positive or negative. Moreover, they show that transfer rate and type of transfer and transfer rate positively associates with model's performance. They define data alignment can be represented using covariance matrix. They show that when the experimental task has similar or the same covariance matrix with the target task, then positive transfer would happen and when the experimental task has different covariance from the target task, negative transfer would happen.

% \subsection{Efficiently Identifying Task Groupings for Multi-Task Learning}
% Our work is built based on the belief that models can learn from other SE tasks who share common knowledge with our targeted task. Therefore, for any pair of SE tasks, there is a way to measure the amount of knowledge sharing among the two tasks. Fifty et al. described the idea of inter-task affinity. They calculate the ratio of lookahead losses where they are before and after the gradient step on the shared parameters as a scale invariant measure of relative progress. They then define inter-task affinity as the average of the sums of 1-losses ratio.

%The SE tasks ca code-to-code (e.g., code translation), code-to-text (e.g., code summarization), and code-to-value (e.g., defect detection).

%fine-tuning of SE pre-trained models
% Source code pre-trained language models have been evaluated and fine-tuned for various SE tasks, demonstrating promising results. Those SE tasks include code-to-code (e.g., code translation), code-to-text (e.g., code summarization), and code-to-value (e.g., defect detection). However, researchers have mostly only looked into fine-tuning one downstream task using a pre-trained model. In our study, we investigate the impact of the order of fine-tuning multiple tasks before the interested target task on its performance. To control and restrict the fine-tuning chain length and the number of permutations so that we can finish the experiments within a reasonable amount of time, we select 4 actively researched SE tasks that are different from each other in terms of using and processing code: Clone Detection (CD), Defect Detection (DD), Code Translation (CT), and Code Repair (CR). Table X provides details on the fine-tuning datasets, language models, evaluation metrics, task definitions, and abbreviations.

==> figures/03-method.tex <==
\section{Experimental Setup}
\label{sec:method}

Our goal was to investigate whether the fine-tuning task orderings of SE tasks have an impact on the performance of the target task (RQ1). Then, we aimed to explore the possible reasons from various dimensions for such an impact (RQ2). Figure \ref{fig:overview} shows a structural view of all the factors we analyzed. Lastly, we aimed to give suggestions for selecting the most cost-effective task orderings for a given target task (RQ3). In the following subsections, we detail the applied experimental setup to answer our research questions. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/sitemap.pdf}
    \caption{Overview of Factors Explored in this Study}
    \label{fig:overview}
\end{figure}

\subsection{Experimental Pipeline}

In this study, we select four downstream SE tasks (CD, DD, CR, and CT) from CodeXGLUE~\cite{lu2021codexglue}, a benchmark dataset for code intelligence. Table \ref{tab:tasks} enumerates the four SE tasks we used in our experiments. We list brief definitions of these selected tasks below:

\noindent{\textbf{Clone Detection (CD)}}
is a task of retrieving similar code given a code snippet as a query. 

\noindent\textbf{Defect Detection (DD)}
is to identify whether a given function is vulnerable or not, which is a binary classification task.

\noindent\textbf{Code Repair (CR)}
aims to automatically repair bugs in the code.

\noindent\textbf{Code Translation (CT)}
aims to translate source code from one programming language to another programming language. In this study, the translation is between Java and C\#.
%fine-tuning chains (i.e. a fine-tuning chain of length 4 means that 4 tasks are fine-tuned sequentially on the pre-trained model. The last task in the chain is our target task of interest, while the fine-tuned tasks before the target task are intermediate tasks.). 

All four tasks are among the widely-used SE tasks for evaluating pre-trained models of source code~\cite{niu2023empirical}. Table \ref{tab:tasks} shows the abbreviation (Ab.), the dataset, and the main evaluation metric. The evaluation metrics and datasets are consistent with those used by CodeXGLUE for each corresponding task. 

The objective of our study is to investigate the impact of task orderings on the performance of different target tasks. We utilize varying numbers of SE tasks within fine-tuning chains, where one to three tasks function as intermediate tasks, sequentially fine-tuned before the target task. 

The target task can be any of the four SE tasks. This results in a total of 60 fine-tuning chain models, with lengths (i.e., the total number of fine-tuning tasks in a chain) varying from 2-4.To ensure comprehensive evaluation, we employ a 10-fold cross-validation technique on a combined dataset of train, dev, and test data from the corresponding task in CodeXGLUE. We establish baseline models for the four tasks by training directly with pre-trained model on the target task datasets. This enables us to determine the statistical significance of any performance disparities between a fine-tuning chain model and a baseline model, facilitating the identification of interesting task ordering patterns. Other settings, including hyper-parameters and the optimizer, are same as CodeXGLUE.

%In our study, we examine the effects of task orderings on the performance of various target tasks. We utilize different numbers of SE tasks within these fine-tuning chains, with any one to three tasks serving as intermediate tasks, fine-tuned in sequence prior to the target task, which can also be any one of the four SE tasks. To ensure a thorough evaluation, we employ a 10-fold cross-validation technique on a combined dataset of train, dev, and test data from the corresponding task in CodeXGLUE. This process allows us to assess the statistical significance of any performance disparities between a fine-tuning chain model and a baseline model, ultimately helping us uncover interesting task ordering patterns.

%Our experiments involve fine-tuning one to three intermediate tasks in all possible permutations, with one remaining task designated as the target task. This results in a total of 60 fine-tuning chain models, with lengths (i.e., the total number of fine-tuning tasks in a chain) varying from 2-4. We also establish baseline models for the four tasks, which are trained directly with pre-trained model on the target task datasets using the same cross validation procedure. Other settings, including hyper-parameters and the optimizer, are consistent with those employed by CodeXGLUE.

Our experiments utilize CodeBERT as the pre-trained encoder for all four tasks. We select CodeBERT because it has been evaluated and compared in many studies~\cite{kanade2020learning,lu2021codexglue,wang2021codet5}. We follow a sequential fine-tuning approach, whereby the encoder is fine-tuned on each intermediate task before proceeding to the target task. For instance, in a task order consisting of four tasks, the encoder is fine-tuned on three intermediate tasks in sequence before being fine-tuned with the target task's dataset. Each task comprises its own unique component or layers. For code generation tasks (CR and CT), we follow CodeXGLUE's setup by employing a randomly initialized Transformer with six layers, 768-dimensional hidden states, and 12 attention heads as the decoder. In the case of CR and CT being part of the same fine-tuning chain, the decoder fine-tuned on one task serves as the starting point for the subsequent task, enabling it to leverage the knowledge accumulated from the previous task. We use softmax layers as task-specific components for classification (DD) and retrieval (CD).

%we employ CodeBERT as the pre-trained encoder for all four tasks. We sequentially fine-tune the encoder on each intermediate task before proceeding to the target task. For instance, in a task ordering consisting of four tasks, the encoder is fine-tuned on three intermediate tasks in sequence before being fine-tuned with the target task's dataset. Furthermore, each task features its own unique component or layers. For code generation tasks, such as CR and CT, we followed CodeXGLUE's setup by using a randomly initialized Transformer with 6 layers, 768 dimensional hidden states and 12 attention heads as the decoder. When CR and CT are part of the same fine-tuning chain, the decoder fine-tuned on one task serves as the starting point for the subsequent task, allowing it to learn the information accumulated from the previous task. For classification (i.e., DD) and retrieval (i.e., CD) tasks, we use softmax layers as their task-specific components.

%\hl{Bad english}To make our findings from the experiments more generalizable, the four selected SE tasks involve various methods of utilizing and manipulating code. As for the pre-trained model in this study, we select CodeBERT because it has been evaluated and compared in many studies~\cite{kanade2020learning,lu2021codexglue,wang2021codet5}. 

To keep the number of experiments manageable, we did not try other pre-trained models of source code or more SE tasks other than the four we picked. We believe this selection is sufficient for us to analyze and explain the general impact of different task orderings on target task performance. In addition, our goal is not to identify the optimal task ordering for a target task fine-tuned with a specific pre-trained model but to investigate task orderings' impacts and the potential factors that may help explain them.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[ht]
% \centering
% \caption{Details of Evaluation Tasks, Datasets, and Metrics}
% \label{tab:tasks}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Type}} & \textbf{Task}    & \textbf{Ab.} & \textbf{Dataset} & \textbf{Language} & \textbf{Metric} \\ \hline
% \multirow{2}{*}{Und.}               & Defect Detection & DD           & Devign           & C                 & Accuracy        \\ \cline{2-6} 
%                                     & Clone Detection  & CD           & POJ-104          & C/C++             & MAP@R           \\ \hline
% \multirow{2}{*}{Gen.}               & Code Repair      & CR           & Bugs2Fix         & Java              & BLEU            \\ \cline{2-6} 
%                                     & Code Translation & CT           & CodeTrans        & Java-C\#          & BLEU            \\ \hline
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
\centering
\caption{Details of Evaluation Tasks, Datasets, and Metrics}
\label{tab:tasks}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Task}    & \textbf{Ab,} & \textbf{Dataset} & \textbf{Dataset Size} & \textbf{Language} & \textbf{Metric} \\ \hline
Defect Detection & DD           & Devign           & 26.4k                 & C                 & Accuracy        \\ \hline
Clone Detection  & CD           & POJ-104          & 52k                   & C/C++             & MAP@R           \\ \hline
Code Repair      & CR           & Bugs2Fix         & 122k                  & Java              & BLEU            \\ \hline
Code Translation & CT           & CodeTrans        & 11.5k                 & Java-C\#          & BLEU            \\ \hline
\end{tabular}%
}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[ht]
% \centering
% \caption{Details of Evaluation Tasks, Datasets, and Metrics}
% \label{tab:tasks}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Type}} & \textbf{Task}    & \textbf{Ab,} & \textbf{Dataset} & \textbf{Dataset Size} & \textbf{Language} & \textbf{Metric} \\ \hline
% \multirow{2}{*}{Und.}               & Defect Detection & DD           & Devign           & 26.4k                 & C                 & Accuracy        \\ \cline{2-7} 
%                                     & Clone Detection  & CD           & POJ-104          & 52k                   & C/C++             & MAP@R           \\ \hline
% \multirow{2}{*}{Gen.}               & Code Repair      & CR           & Bugs2Fix         & 122k                  & Java              & BLEU            \\ \cline{2-7} 
%                                     & Code Translation & CT           & CodeTrans        & 11.5k                 & Java-C\#          & BLEU            \\ \hline
% \end{tabular}%
% }
% \end{table}

% \subsection{Selection of Datasets}
% We obtained the fine-tuning datasets for all 4 selected tasks from CodeXGLUE. For CD, we picked the POJ104 retrieval dataset using C/C++ as the programming language. For DD, we picked the Devign dataset, a classification Dataset using C as the programming language. We used the Bugs2Fix dataset using java as the programming language for CR. We used the CodeTrans dataset using java-C\# as the programming language for CT. Note that CR and CT are generative tasks, so their dataset contains two parts: input and output. Therefore, CR's datasets are: CR\_BUGS2FIX\_Input, CR\_BUGS2FIX\_Output, and CT's datasets are: CT\_CODETRANS\_Input, and CT\_CODETRANS\_Output.


\subsection{Analyses of Dataset Characteristics}

Next, we analyze various characteristics of the training dataset in order to explain the impact on performance. The characteristics we selected have been used in NLP research for analyzing the positive transfer learning between a variety of downstream tasks~\cite{vu2020exploring,chang2021rethinking}.
%. Since training dataset always plays a vital role in machine learning, considering the characteristics of a dataset to explain this impact becomes reasonable, as they have also been considered in NLP research analyzing the positive transfer learning conditions between a variety of downstream tasks~\cite{vu2020exploring,chang2021rethinking}.

% \noindent\textit{\textbf{Dataset Domain Similarity: }}Vu et al.~\cite{vu2020exploring} showed that the similarity of training data domains may influence the efficacy of transfer learning between NLP tasks. To describe the data domain from a pre-trained language model's learning perspective, they developed a method utilizing BERT token-level representations of inputs across the entire dataset. Specifically, they passed each input sample through the pre-trained BERT model~\cite{devlin2018bert} without fine-tuning and computed the average of the final layer token-level representations. The resulting text embedding (TEXTEMB) is the average of these pooled hidden vectors for the entire dataset. The authors posited that this method could capture the linguistic properties of both the input text and the entire dataset. To assess domain similarity, they calculated cosine similarity between TEXTEMBs of the intermediate and target task datasets. They concluded that TEXTEMB is a reliable predictor of successful transfer.

% In our research, we adapt this method to evaluate domain similarities among various SE task-specific datasets. The only difference from Vu et al.'s~\cite{vu2020exploring} approach was that we use CodeBERT~\cite{feng2020codebert} instead of BERT to produce token-level representations for all code snippets in task-specific datasets. \hl{Isn't Vu suing BERT and we are using CodeBERT? seems written opposite} We averaged the representations to generate TEXTEMBs for all four datasets in our experiments and computed the cosine similarities for all TEXTEMB pairs. As CodeBERT's maximum input token sequence length is 512, we created TEXTEMBs for code snippets in all datasets in two ways: (1) \textbf{\textit{Truncation:}} we truncate tokens exceeding the limit, and (2) \textbf{\textit{Split:}} we split the token sequence into multiple sequences, each with a token count less than or equal to 512. This sequence split would cause the total number of sequences to increase (i.e. we would have extra two more sequences after spliting a long sequence into three parts). Therefore, we use this increased total number of sequences when calculating TEXTEMB. \hl{what does the last senetence mean?}

\noindent\textit{\textbf{Syntactic Similarity Analysis: }} Ahmed et al.~\cite{ahmed2022multilingual} have shown that the language model's performance on downstream SE tasks can be improved by utilizing shared syntactic information between datasets consisting of code snippets with similar purposes but written in different programming languages. Motivated by this, we explore the syntactic similarities of datasets by focusing on three code-related characteristics: \textit{keywords}, \textit{operators}, and \textit{identifiers}. However, analyzing all possible pairs of programs from each dataset pair would be unfeasible due to the large size of each dataset. Thus, we choose to utilize a sampling approach to reduce the size. We determine the appropriate sample size for each dataset with a confidence level of 99\% and a margin of error of 2\% and then proceed to analyze the resulting sampled dataset.

We calculate the similarity following the procedure below:

(1) We randomly sample datasets using the calculated sample size. 

(2) Every dataset consists of code snippets. We go through the sampled dataset and gather information on the keywords, operators, and identifiers of each code snippet.

(3) We loop through the combination that contains pairs of code snippets selected from each pair of datasets. For every pair of code snippet, we apply the Jaccard similarity formula(J = $ \frac{|A \cap B|}  {|A \cup B|} $ where A and B two sets)~\cite{niwattanakul2013using} to calculate their similarities in terms of the keywords, operators, and identifiers. 

 (4) After computing the similarity scores for each pair of code snippets, we calculate the overall similarity of the two datasets by taking the average similarity across all code snippets.

\noindent\textit{\textbf{Semantic Similarity Analysis: }}
After examining the syntactic similarities,  we shift our attention to analyzing semantic similarity among datasets. To extract the semantic information of a code snippet, we conduct feature extraction using CodeBERT since the pre-trained CodeBERT model can provide a reliable vector representation containing the code snippets' semantic information~\cite{feng2020codebert}.
%After examining the syntactic similarities of datasets from the keywords, operators, and identifiers perspectives, we recognize that the content of the code snippets can impact model learning. In this analysis, we shift our attention from analyzing syntactic similarity to semantic similarity among datasets. To extract the semantic information of a code snippet, we conduct feature extraction using CodeBERT. Since pre-trained CodeBERT model can provide us with a reliable vector representation containing the code snippets' semantic information~\cite{feng2020codebert}.

Our approach involves employing the CodeBERT model to obtain vector representations for code snippets. We then evaluate the semantic similarity between the pair of code snippets from two datasets by computing the cosine similarity~\cite{rahutomo2012semantic}. Ultimately, we utilize the similarity scores obtained from all pairs of code snippets from both datasets to determine the semantic similarity between the two datasets. Specifically, we average the cosine similarities for all pairs of code snippets from the two datasets to calculate the semantic similarity of the two datasets.

Due to the enormous size of each dataset, analyzing all possible pairs of code snippets from each dataset would be a daunting task. Thus, we resort to sampling. To determine the appropriate sample size for each dataset, we utilize the same sample size calculator with a 99\% confidence level and a 2\% margin of error. Subsequently, we sample each dataset using the population size calculated by the sample size calculator. Our analysis steps are the following:

(1) We select two datasets and then proceed to sample them using the previously calculated sample size.

(2) For each pair of datasets, we loop through their combinations which is a set of pairs of code snippets. 

(3) To generate vector representations for both code snippets, we use CodeBERT. However, CodeBERT has a constraint on the number of input tokens which is 512. For code snippets with more than 512 tokens, we split them into multiple parts, each containing a maximum of 512 tokens. After that, we construct vector representations for each part and concatenate them all. This way, we get the vector representation of the code snippet. 

(4) We determine the semantic similarity between the two code snippets using the cosine similarity between their vector representations. We repeat this step for every pair of code snippets in the combination. We then determine the semantic similarity of the two datasets by averaging the cosine similarity scores across all pairs of code snippets.

(5) We repeat the previously described steps for all pairs of datasets.



% \hl{what is code program??: change to source code program}
% \hl{Spellcheck and consistency check of the term CodeBERT: done}
% \noindent\textit{\textbf{Covariance Matrix Analysis: }}In a study by Wu et al.~\cite{wu2020understanding}, it was found that the alignment of data for tasks can greatly impact the performance of a deep learning model in multi-task learning. Although our training method is not identical to multi-task learning, the parameters of the encoder and decoder are updated through a similar shared parameter mechanism. Therefore, it is valuable to examine the data alignment of the datasets used in our study. It's important to note that this analysis is symmetrical because it concentrates on differences in the data distribution of both datasets.


% We assert that the covariance matrix analysis we employ is distinct from common program analysis and syntactic similarity analysis. While common program analysis emphasizes the semantic information of each program and syntactic analysis concentrates on the syntactic information of each program, our analysis concerns the geometric arrangement of the data samples in high-dimensional space as represented by their vector representations.

% In specific, our analysis step is the following:
% \begin{itemize}
%     \item We generate vector representations for each source code program in each dataset. However, since CodeBERT has a token limit of 512, for scripts with more than 512 tokens, we divide them into multiple groups, each with a maximum of 512 tokens. Subsequently, we create vector representations for each group and then concatenate them to obtain the vector representation of the entire program. 
%     \item By considering the vector representation of each source code program as a data point in high-dimensional space, we construct the covariance matrix for the dataset with the help of numpy. This covariance matrix characterizes the distribution of the source code programs in the dataset.
%     \item We use the Frobenius Norm formula to compute the distance between the covariance matrices of two datasets, which reflects their data alignment. This step is repeated for all dataset pairs. The Frobenius Norm formula is represented by d = 1- $\frac{tr(R_1 * R_2)}{\lVert{R_1}\rVert * \lVert{R_2}\rVert }$, where $R_1 and R_2$ are the covariance matrices.
% \end{itemize}


%Following Vu et al.'s approach~\cite{vu2020exploring} of examining the impact of training data size on the transferability between NLP tasks, we perform experiments with 4 data regimes to investigate the impact of training data size on the transferability between SE tasks, namely \textit{FULL to FULL}, \textit{FULL to LIMITED}, \textit{LIMITED to FULL}, \textit{LIMITED to LIMITED}. In the FULL data setting, all available training data for an SE task is used for fine-tuning, while only 1K training data points are randomly sampled from the whole training dataset in the LIMITED regime. We should note that the chains fine-tuned with \textit{FULL to FULL} and \textit{LIMITED to FULL} data regimes can be readily compared with our baselines trained in Section \ref{} (\textit{FULL} baseline), while we additionally trained corresponding \textit{LIMITED} baselines by directly training the pre-trained model with the \textit{LIMITED} target task data. Since chains trained in \textit{FULL to LIMITED} and \textit{LIMITED to LIMITED} data regimes have the target tasks trained with \textit{LIMITED} data, it would be reasonable to compare their performances with that of \textit{LIMITED} baseline rather than \textit{FULL} baseline. In this study, we only conduct this experiment on the interested fine-tuning chain patterns with the goal of explaining why such patterns always boost or hurt the performance of the target task. 

\noindent\textit{\textbf{Dataset Size Analysis:}} Many research works in NLP have explored the influence of both intermediate and target dataset sizes on the performance of target tasks. These investigations found that target tasks with smaller datasets gained the most from intermediate task training in general. However, they discovered no significant, consistent effect of intermediate task dataset size on the performance of target tasks. Instead, they highlighted the importance of other factors for positive transfer between certain NLP tasks~\cite{phang2018sentence, vu2020exploring, pruksachatkun2020intermediate, chang2021rethinking}. In our study, we briefly examined the potential role of training dataset size in explaining the varying impacts of specific fine-tuning task orderings on target task performance. %using the four SE tasks and their datasets provided by CodeXGLUE.
\subsection{Analyses of SE Task Characteristics}
\label{sec:SE task sim}
\noindent\textit{\textbf{Task Affinity Analysis:}}
Based on the study by Fifty et al.~\cite{fifty2021efficiently}, the level of task affinity between two tasks can reveal the extent to which one task can benefit another task. In other words, it can indicate how much knowledge can be transferred between the two tasks. Given that our training approach updates weights based on the SE tasks in the task orderings, we posit that task affinity is a crucial factor in determining the models' performance.

% Multi-task learning consists of a shared module and task-specific modules. The shared module's weights are updated based on the loss that is the linear combination of sublosses of all tasks. As a result, the quality of the shared module is critical in determining the model's performance and is heavily dependent on the suitability of the involved tasks. To measure the quality of knowledge sharing among tasks, Fifty et al.~\cite{fifty2021efficiently} have proposed task affinity, which indicates the usefulness of one task for another. Therefore, it is crucial to examine the compatibility of the tasks during training. \hl{rewrite this para. First, why are we starting by talkin g about Multi-task learning? second, it doesn't really say anything about what is task affinity. Rewrite by simply saying what is task affinity}

The aim of this analysis is to investigate the task affinity between tasks. We define \textit{intermediate fine-tuned model}: The fine-tuning chain model where the pre-trained model is fine-tuned with the intermediate tasks in the task orderings without the target task, which is the starting point for the target task to train on. For example, for task ordering CR$\rightarrow$CT, intermediate fine-tuned model would be the CR baseline model.

% In each training path, we consider the last task as the target task. We use CodeBERT for the encoder and Roberta for the decoder as our default model. The perfect model \hl{what is perfect model? this is the first time I am seeing this term}is obtained by training the default model on the target task. On the other hand, the path model results from training all tasks in the chain, except for the target task.\hl{rewrite this para. It is not following the same style of writing as the previous characterisitcs}

We start by training the pre-trained, baseline, and intermediate fine-tuned models on the target task, and record their losses. Then, we calculate the sum of the differences in losses between the intermediate fine-tuned and baseline models, which we label as diff\_intermediate. Similarly, we calculate the sum of the loss differences between the pre-trained and baseline models, known as diff\_pre-trained. As an example, suppose the task ordering is CR$\rightarrow$CT, the intermediate fine-tuned model would be the baseline CR model and the target task would be CT. We train the pre-trained model with CT dataset, record the losses and label it as pre-trained\_loss. We then train the intermediate fine-tuned model with CT dataset, record the losses and label it as intermediate\_loss. We lastly train the CT baseline model again with CT dataset, record the losses and label it as baseline\_loss. Thus, the diff\_intermediate equals sum of differences between intermediate\_loss and baseline\_loss. The diff\_pre-trained equals sum of differences between pre-trained\_loss and baseline\_loss.

We then compare diff\_intermediate with diff\_pre-trained to determine the effectiveness of knowledge transfer from intermediate tasks to the target task, which is the task affinity. We should note that this analysis is asymmetric because, for any task ordering, we compare the intermediate fine-tuned model with its baseline model. We consider this method valid because we use the baseline model's losses on the target task as a reference point for comparison. Compared to pre-trained model and intermediate fine-tuned model, baseline model is the only model who has been trained on the target task. Therefore, when retraining it on the target task, its losses on the target task would be the ideal case, and by comparing diff\_pre-trained and diff\_intermediate, we would tell the model that is closer to the baseline model, which explains whether the intermediate tasks help transfer knowledge.

% It is worth noting that smaller losses for the pre-train or intermiedate fine-tuned models do not necessarily indicate positive task affinity. To address this issue, we utilize the baseline model as a reference point for comparisons. \hl{m,any problems. Why can't we use the previous works definition of affinity? if we can then we don't need all these explanations regarding how we did it. If we cannot use the previous def, then we need to explain why our definition makes sense}


% \noindent\textit{\textbf{Classification VS Retrieval: }}In our research, we have observed that the SE tasks we used can be categorized as either understanding (CD, DD) or generation (CR, CT), where understanding tasks involve retrieval and classification. For our study, we selected the POJ104 and DEVIGN datasets for the CD and DD tasks, respectively, and created a converted classification POJ104 dataset to explore whether task type affects the model's performance. To avoid the differences in the programming languages and code snippet domains between BCB and POJ104,\hl{what is that? no idea what is datset content bias: resolved} we did not use the BCB dataset provided by CodeXGlue. Furthermore, since the DEVIGN dataset is in C and the BCB dataset is in Java, we constructed our classification dataset from the POJ104 dataset to eliminate the language difference. Note that we were unable to create a retrieval dataset for DD due to the absence of paired information in the defeat detection dataset.

% % Converted CD dataset construction
% To construct our classification CD dataset, we started with the POJ104 retrieval dataset. Each data instance in the POJ104 dataset includes label, index, and code fields, where the label indicates the group to which the code belongs, and the index is the source code index. We took advantage of the fact that data instances in the same group are clones of each other, as stated in the CodeXGlue paper. To create a classification dataset, we crafted two instances for each example in the POJ104 dataset, one for clone and one for not clone. To do this, we randomly selected another instance in the same group to create a clone sample \hl{what is postive sample: resolved}for every example. To build a non-clone sample\hl{what is negative sample?: resolved}, we randomly selected an instance from a different group number. We repeated the random selection process if there was any duplication. Thus, we generated a converted classification CD dataset comprising 64,000 training data points with an equal distribution of 50\% clone and 50\% non-clone examples. Furthermore, to ensure the data balance between our converted dataset and the DEVIGN dataset, we evaluated the data balance of the DEVIGN dataset and found that it consists of 50\% defeat and 50\% non-defeat data samples. \hl{why? is DD balanced?: resolved}

% In our analysis, we trained the model on four different types of paths.
% \begin{itemize}
%     \item Type 1: All paths where DD is the last task and CD exists in the paths. When training those paths, we use our classification CD dataset and the classification DD dataset. 
%     \item Type 2: All paths where CD is the last task and DD exists in the paths. When training those paths, we use our classification CD dataset and the classification DD dataset. 
%     \item Type 3: All paths where DD is the last task and CD exists in the paths. When training those paths, we use retrieval CD dataset and classification DD dataset.
%     \item Type 4: All paths where CD is the last task and DD exists in the paths. When training those paths, we use retrieval CD dataset and classification DD dataset.
% \end{itemize}



% Below we summarize the detail of two comparisons 
% \begin{itemize}
%     \item \textbf{Type1 VS Type3}: The task ordering is CD$\rightarrow$DD. This comparison helps understand how classification CD and retrieval CD can impact the performance of DD because the target task DD is classification, and CD can be either classification and retrieval. 
%     \item \textbf{Type2 VS Type4}: The task ordering is DD$\rightarrow$CD. Cannot be compared because the target task CD employs two different metrics, namely F1 for classification and MAP@R for retrieval.
% \end{itemize}


% \begin{table}[ht]
% \caption{Task Type Comparison Detail Table}
% \label{tab:cd-dd-type}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Comparisons}    & \textbf{Datasets involved}   & \textbf{Detail}  \\ \hline
% Type1 VS Type3          & Classification CD$\rightarrow$Classification DD VS Retrieval CD$\rightarrow$ Classification DD   &    This comparison can help us understand how task type of CD can impact the performance of DD.                        \\ \hline
% Type2 VS Type4          & Classification DD$\rightarrow$Retrieval CD VS Classification DD$\rightarrow$Classification CD    &   Cannot be compared because even they employ different metrics. Classification CD in type 2 uses F1, while retrieval CD in type 4 uses MAP@R.
%                                         \\ \hline   
% \end{tabular}%
% }
% \end{table}
% \hl{this is difficult to parse. Why don't you simply create a table?}
% Once we have trained all groups, we compare the performance of type 1 path and type 3 path who both end with classification DD model. This comparison can help us understand how task type of CD can impact the performance of DD. It's worth mentioning that we deliberately exclude the comparison between type 2 and 4 paths because even they both contain CD as the target task, their CDs are two different types and employ different metrics. Classification CD in type 2 uses F1, while retrieval CD in type 4 uses MAP@R. 

% \noindent\textit{\textbf{Understanding VS Generation: }}SE tasks have been classified into two general categories, code understanding (Und.) or code generation (Gen.), by previous study~\cite{niu2022deep}. In this work, we have two tasks that fall into each of the two categories, that is, DD and CD are code understanding tasks while CR and CT are code generation tasks. We aim to investigate whether the task category could be a factor that helps explain why certain orders of intermediate tasks can boost or degrade the performance of the target task.

\subsection{Analyses of Model Characteristics}
\label{sec:modelanalysis}

\noindent\textit{\textbf{Probing Tasks Analysis: }}Having a good performance on an SE task usually requires the model have a good understanding of some code properties. In this study, we posit that models fine-tuned with different task-specific datasets may exhibit different extents of understandings of a certain code property, and the fine-tuning of some intermediate tasks can affect the target task's learning of a code property critical for the model to perform well on  target task.
%. For example, the performance gain of a target task in a fine-tuning chain model could be due to the fact that some intermediate task increases the model's understanding of a code property, which is critical for the model to perform well on this target task.

To evaluate the acquisition of language skills learned by a model, researchers have come up with \textit{probing tasks}. These tasks are diagnostic in nature, where a simple linear classifier is trained on the vector embeddings of a language model to predict specific properties of its input (i.e. natural language texts). The performance of the classifier on probing tasks indicates whether probed information exists in the vector embedding of a model and the extent to which such information is encoded or learned. Probing has been extensively designed and studied for models trained with natural language with the aim of analyzing a large amount of natural language properties and skills~\cite{adi2016fine, alain2016understanding, belinkov2017neural, conneau2018you, tenney2019you}.

In a more recent time, probing tasks from NLP have been adapted to pre-trained language models of source code. Various probing tasks have been constructed to evaluate the hidden vectors of a model and their ability to grasp code-related characteristics after model pre-training stage~\cite{karmakar2021pre, troshin2022probing, wan2022they}. These code-related characteristics may be useful in downstream SE tasks. In our study, we use two of the probing tasks from \cite{karmakar2021pre} to assess the models' learning degrees of source code semantic and syntactic information. The probing task that is designed for testing the model's syntactic understanding of source code is Abstract Syntax Tree Node Tagging (AST), which is a task of identifying AST node tags for a sequence of code tokens. Another one that is for assessing the model's awareness of code semantics is Invalid Type Detection (TYP). The model is asked to distinguish between code snippets that contain misspelled primitive data types from semantically valid ones. 

In this study, we train a logistic regression classifier~\cite{lavalley2008logistic} (the hyper-parameters are set the same as those from \cite{karmakar2021pre}) that takes the input feature vectors from the frozen hidden layers of fine-tuning chain models. The accuracy's are based on the vector embeddings from each of the hidden layers in CodeBERT ranging from 1-12. Pre-trained CodeBERT has been probed to have heterogeneous probing task performance across layers~\cite{karmakar2021pre}. To evaluate the general understanding of a particular probed skill from a fine-tuned model, we take the average of all 12 accuracy's (from all 12 layers) as an estimate of the model's overall performance. We call this average the \textit{probing task performance} for a fine-tuned model in the following sections. Next, we investigated the relationship between probing and target tasks in order to see whether a probed code-related skill is important for a fine-tuned model to perform well on this target task. The \textit{target task performance} is the average of the performances of all 10-fold cross validation models. Similar to \cite{pruksachatkun2020intermediate}, we calculate the Spearman correlation~\cite{myers2004spearman} between probing task and target task performances for all fine-tuning chain models whose task orderings end with the target task. With the knowledge of different SE tasks' requirements for the probed skills, we finally provide insights into why certain task orderings boost or hurt the target task performance (i.e. positive transfer or negative transfer) by comparing the performances of probing tasks.

\noindent\textit{\textbf{Attention Analysis: }}In this study, we investigate the attention weight assignments of CodeBERT's heads on different syntax tokens in its input sequence. CodeBERT is a transformer-based model that generates self-attention weights for each token in the input sequence. These weights are an indicator of the level of attention that other tokens in the input sequence give to each token. CodeBERT consists of 12 self-attention layers, with each layer having 12 heads that produce attention weights for the same token. To obtain a comprehensive measure of the attention weight for each token, we average the attention weights across all layers and heads.

To analyze the attention weights assigned by CodeBERT's heads, we consider different versions of the fine-tuned model and assess the salience of various syntax tokens, including identifiers, modifiers, operators, data types, separators, keywords, strings, and Booleans. These syntax tokens were selected based on prior work by Aljehane et al.~\cite{aljehane2021determining}. We extract these syntax tokens from the input source code using Javalang~\cite{javalang}, a widely used Java syntax collection library. Additionally, we investigate the role of abstract syntax structures, such as method signature, if-else statements, while statements, and return statements, in determining the attention behavior of fine-tuned CodeBERT. To identify these abstract syntax tree structures, we utilize tree-sitter-java~\cite{tree-sitter}, a commonly used Java abstract syntax tree structure identification library.

\subsection{Analysis of Time and Performance}
% In our study, we evaluated all possible combinations of paths for the four tasks \hl{upto this point we haven't disclosed that we are doing for 4, so don't dosclos enow}and recorded the time each path took. 
\label{sec:timeanalysis}
Training deep learning models on SE tasks consumes relatively large amount of hardware and time resources.~\cite{strubell2020energy, strubell2019energy}. This training time can vary from a few hours to hundreds of hours. When selecting the task ordering for a given target task, the performance should not be the only factor to consider, but also the resources it consumes. 

In this analysis, we aim to answer RQ3, which focuses on considering the time-performance trade-offs to pick the optimal task ordering for performance improvement. We examine all the task orderings of positive transfer and compare the model performance gain with the additional training time required. Specifically, we estimate the model performance gain by using \textit{relative performance gain} from~\cite{vu2020exploring}, which is defined as $$g_{fine-tuning\_chain\_model} = \frac{P_{fine-tuning\_chain\_model} - P_{baseline}}{P_{baseline}}$$  where $P_{baseline}$ represents baseline model performance and\\ 
$P_{fine-tuning\_chain\_model}$ represents the performance of the fine-tuning chain model with the same target task. Furthermore, in order to  analyze the cost-effectiveness of each task ordering, we define \textit{effective ratio} as 


% below two are exactly same and first is buggy, use second 
% $$\bm{\mathit{\Delta}} $$
% $$\mathit{\Delta}$$

$$effective\_ratio = \frac{g_{fine-tuning\_chain\_model}}{\mathit{\Delta}training\_time} \; $$

Where ${\mathit{\Delta}training\_time}$ represents the training time difference between baseline model and the fine-tuning chain model with the same target task. The effective ratio provides an intuitive way of understanding the cost of performance improvement, namely performance improvement per unit of time.
% $\frac{g_{fine-tuning\_chain\_model}}{\bm{\mathit{\Delta}} training\_hours}$



==> figures/04-results.tex <==
\section{Evaluation Results of Model Performances}
\label{sec:results}

In order to answer our RQ1 about whether task ordering matters, we fine-tune all permutations of four tasks sequentially on CodeBERT. For each fine-tuning chain model whose task ordering ends with a target task, we report its metric score and compare the score with the performance of its baseline model. %By comparing the performances of fine-tuning chain models with their corresponding baseline models, we collect the positive transfer and negative transfer task orderings and further investigate whether there are certain task ordering patterns emerging. 
Given that there are four tasks, the total number of chain models with varying lengths of task orderings is 60. Since we trained the models with 10-fold cross validation, we conduct Welch’s t-test~\cite{ruxton2006unequal} to measure the statistical significance of the performance difference between fine-tuning chain models and baselines to identify whether the chain model is a positive or negative transfer. We show the results in Table \ref{tab:chain-performances}. We also highlight the positive transfer and negative transfer for each model. Based on our results, several interesting patterns emerge. For example, the performances of CD and DD almost always dropped by intermediate task fine-tuning no matter what the intermediate tasks are, while the different task orderings of CR and CT could bring either performance gain or loss. Due to space constraints, in this paper we select two patterns whose task orderings can be both positive and negative transfer depending on the task orderings.

%(2) CD’s performance is mostly always \textit{hurt} by fine-tuning other tasks before it.

\textbf{Pattern 1 (positive transfer ``+'')} When CR is fine-tuned before CT (CR$\rightarrow$CT), CT’s performance becomes statistically significantly \textit{better} than CT baseline. Other intermediate tasks that are fine-tuned between CR and CT in the task orderings of fine-tuning chain models \textit{do not} affect this positive transfer and statistical significance.

\textbf{Pattern 2 (negative transfer``-'')} When CT is fine-tuned before CR (CT$\rightarrow$CR ), CR’s performance becomes statistically significantly \textit{worse} than CR baseline. Other intermediate tasks that are fine-tuned between CT and CR \textit{do not} affect this negative transfer and statistical significance.

%\hl{these 3 patterns are written in different styles. Needs to be in a consistent way so that people can see pattern}

% \begin{center}
%     \begin{tabular}{| l | l | l |}
%     \hline
%     \multicolumn{3}{|c|}{CD Table} \\
%     \hline
%     \textbf{Task\_Path}      &   \textbf{Avg\_Score(MAP@R)}               &       \textbf{Is\_Better?} \\
%         \hline
%     CD              &   0.869                           &       /  \\
%         \hline
%     CT->CR->CD      &   0.847                           &       N* \\
%         \hline
%     CT->CD          &   0.871                           &       Y  \\
%         \hline
%     CR->CT->CD      &   0.862                           &       N  \\
%         \hline
%     CR->CD          &   0.853                           &       N* \\
%         \hline
%     DD->CR->CD      &   0.855                           &       N* \\
%         \hline
%     DD->CD          &   0.853                           &       N* \\
%         \hline
%     CR->DD->CD      &   0.854                           &       N* \\
%         \hline
%     DD->CT->CD      &   0.855                           &       N* \\
%         \hline
%     CT->DD->CD      &   0.866                           &       N* \\
%         \hline
%     DD->CT->CR->CD  &   0.844                           &       N* \\
%         \hline
%     DD->CR->CT->CD  &   0.853                           &       N* \\
%         \hline
%     CT->DD->CR->CD  &   0.841                           &       N* \\
%         \hline
%     CT->CR->DD->CD  &   0.854                           &       N* \\
%         \hline
%     CR->DD->CT->CD  &   0.857                           &       N* \\
%         \hline
%     CR->CT->DD->CD  &   0.856                           &       N* \\
%         \hline
%     \hline
%     \end{tabular}
% \end{center}

% \begin{table}[]
% \caption{CD}
% \label{tab:cd}
% \begin{tabular}{|l|l|l|}
% \hline
% Fine-tuning Chains                                    & \textbackslash{}textbf\{Avg\_Score(MAP@R)\} & \textbackslash{}textbf\{Is\_Better?\} \\ \hline
% CD                                                    & 0.869                                       & /                                     \\ \hline
% CT-\textgreater{}CR-\textgreater{}CD                  & 0.847                                       & N*                                    \\ \hline
% CT-\textgreater{}CD                                   & 0.871                                       & Y                                     \\ \hline
% CR-\textgreater{}CT-\textgreater{}CD                  & 0.862                                       & N                                     \\ \hline
% CR-\textgreater{}CD                                   & 0.853                                       & N*                                    \\ \hline
% DD-\textgreater{}CR-\textgreater{}CD                  & 0.855                                       & N*                                    \\ \hline
% DD-\textgreater{}CD                                   & 0.853                                       & N*                                    \\ \hline
% CR-\textgreater{}DD-\textgreater{}CD                  & 0.854                                       & N*                                    \\ \hline
% DD-\textgreater{}CT-\textgreater{}CD                  & 0.855                                       & N*                                    \\ \hline
% CT-\textgreater{}DD-\textgreater{}CD                  & 0.866                                       & N*                                    \\ \hline
% DD-\textgreater{}CT-\textgreater{}CR-\textgreater{}CD & 0.844                                       & N*                                    \\ \hline
% DD-\textgreater{}CR-\textgreater{}CT-\textgreater{}CD & 0.853                                       & N*                                    \\ \hline
% CT-\textgreater{}DD-\textgreater{}CR-\textgreater{}CD & 0.841                                       & N*                                    \\ \hline
% CT-\textgreater{}CR-\textgreater{}DD-\textgreater{}CD & 0.854                                       & N*                                    \\ \hline
% CR-\textgreater{}DD-\textgreater{}CT-\textgreater{}CD & 0.857                                       & N*                                    \\ \hline
% CR-\textgreater{}CT-\textgreater{}DD-\textgreater{}CD & 0.856                                       & N*                                    \\ \hline
% \end{tabular}
% \end{table}


% \begin{center}
%     \begin{tabular}{| l | l | l |}
%     \hline
%     \multicolumn{3}{|c|}{DD Table} \\
%     \hline
%     \textbf{Task\_Path}      &   \textbf{Avg\_Score(Accuracy)}               &       \textbf{Is\_Better?} \\
%     \hline
%     DD              &       0.630                       &    /  \\
%     \hline
%     CR->DD          &       0.626                       &    N  \\
%     \hline
%     CR->CD->DD      &       0.610                       &    N* \\
%     \hline
%     CD->DD          &       0.619                       &    N* \\
%     \hline
%     CD->CR->DD      &       0.626                       &    N  \\
%     \hline
%     CT->DD          &       0.628                       &    N  \\
%     \hline
%     CT->CD->DD      &       0.610                       &    N* \\
%     \hline
%     CD->CT->DD      &       0.628                       &    N  \\
%     \hline
%     CT->CR->DD      &       0.621                       &    N  \\
%     \hline
%     CR->CT->DD      &       0.627                       &    N  \\
%     \hline
%     CT->CR->CD->DD  &       0.605                       &    N* \\
%     \hline
%     CT->CD->CR->DD  &       0.614                       &    N* \\
%     \hline
%     CR->CT->CD->DD  &       0.607                       &    N* \\
%     \hline
%     CR->CD->CT->DD  &       0.619                       &    N* \\
%     \hline
%     CD->CT->CR->DD  &       0.606                       &    N* \\
%     \hline
%     CD->CR->CT->DD  &       0.615                       &    N* \\
%     \hline
%     \end{tabular}
% \end{center}

% \begin{table}[]
% \caption{dd}
% \label{tab:dd}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbackslash{}textbf\{Task\_Path\}                  & \textbackslash{}textbf\{Avg\_Score(Accuracy)\} & \textbackslash{}textbf\{Is\_Better?\} \\ \hline
% DD                                                    & 0.630                                          & /                                     \\ \hline
% CR-\textgreater{}DD                                   & 0.626                                          & N                                     \\ \hline
% CR-\textgreater{}CD-\textgreater{}DD                  & 0.610                                          & N*                                    \\ \hline
% CD-\textgreater{}DD                                   & 0.619                                          & N*                                    \\ \hline
% CD-\textgreater{}CR-\textgreater{}DD                  & 0.626                                          & N                                     \\ \hline
% CT-\textgreater{}DD                                   & 0.628                                          & N                                     \\ \hline
% CT-\textgreater{}CD-\textgreater{}DD                  & 0.610                                          & N*                                    \\ \hline
% CD-\textgreater{}CT-\textgreater{}DD                  & 0.628                                          & N                                     \\ \hline
% CT-\textgreater{}CR-\textgreater{}DD                  & 0.621                                          & N                                     \\ \hline
% CR-\textgreater{}CT-\textgreater{}DD                  & 0.627                                          & N                                     \\ \hline
% CT-\textgreater{}CR-\textgreater{}CD-\textgreater{}DD & 0.605                                          & N*                                    \\ \hline
% CT-\textgreater{}CD-\textgreater{}CR-\textgreater{}DD & 0.614                                          & N*                                    \\ \hline
% CR-\textgreater{}CT-\textgreater{}CD-\textgreater{}DD & 0.607                                          & N*                                    \\ \hline
% CR-\textgreater{}CD-\textgreater{}CT-\textgreater{}DD & 0.619                                          & N*                                    \\ \hline
% CD-\textgreater{}CT-\textgreater{}CR-\textgreater{}DD & 0.606                                          & N*                                    \\ \hline
% CD-\textgreater{}CR-\textgreater{}CT-\textgreater{}DD & 0.615                                          & N*                                    \\ \hline
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[]
% \centering
% \caption{The Performances of Fine-tuning Chain Models and Baselines whose Target Tasks are CT)}
% \label{tab:chain-performancesct}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Chain Models}                           & \textbf{Average BLEU Scores} & \textbf{Positive Transfer?} \\ \hline
% CT                                                    & 70.881                       & /                             \\ \hline
% CR$\rightarrow$CT                                   & 74.242                       & Y* \tablefootnote{* represents statistical significance}                            \\ \hline
% CR$\rightarrow$CD$\rightarrow$CT                  & 73.957                       & Y*                            \\ \hline
% CD$\rightarrow$CT                                   & 70.879                       & N                             \\ \hline
% CD$\rightarrow$CR$\rightarrow$CT                  & 75.058                       & Y*                            \\ \hline
% DD$\rightarrow$CT                                   & 70.839                       & N                             \\ \hline
% DD$\rightarrow$CD$\rightarrow$CT                  & 70.739                       & N                             \\ \hline
% CD$\rightarrow$DD$\rightarrow$CT                  & 71.000                       & Y                             \\ \hline
% DD$\rightarrow$CR$\rightarrow$CT                  & 74.113                       & Y*                            \\ \hline
% CR$\rightarrow$DD$\rightarrow$CT                  & 74.118                       & Y*                            \\ \hline
% DD$\rightarrow$CR$\rightarrow$CD$\rightarrow$CT & 73.942                       & Y*                            \\ \hline
% DD$\rightarrow$CD$\rightarrow$CR$\rightarrow$CT & 73.950                       & Y*                            \\ \hline
% CR$\rightarrow$DD$\rightarrow$CD$\rightarrow$CT & 74.145                       & Y*                            \\ \hline
% CR$\rightarrow$CD$\rightarrow$DD$\rightarrow$CT & 73.882                       & Y*                            \\ \hline
% CD$\rightarrow$DD$\rightarrow$CR$\rightarrow$CT & 74.606                       & Y*                            \\ \hline
% CD$\rightarrow$CR$\rightarrow$DD$\rightarrow$CT & 74.204                       & Y*                            \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{table}[t]
% \centering
% \caption{The Performances of Fine-tuning Chain Models and Baselines whose Target Tasks are CR)}
% \label{tab:chain-performancescr}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Chain Models}                           & \textbf{Average BLEU Scores} & \textbf{Positive Transfer?} \\ \hline
% CR                                                    & 79.566                       & /                             \\ \hline
% CT$\rightarrow$CR                                   & 76.824                       & N*                            \\ \hline
% CT$\rightarrow$CD$\rightarrow$CR                  & 77.870                       & N*                            \\ \hline
% CD$\rightarrow$CT$\rightarrow$CR                  & 77.455                       & N*                            \\ \hline
% CD$\rightarrow$CR                                   & 79.643                       & Y                             \\ \hline
% DD$\rightarrow$CR                                   & 79.712                       & Y                             \\ \hline
% DD$\rightarrow$CD$\rightarrow$CR                  & 79.825                       & Y                             \\ \hline
% CD$\rightarrow$DD$\rightarrow$CR                  & 79.616                       & Y                             \\ \hline
% DD$\rightarrow$CT$\rightarrow$CR                  & 77.347                       & N*                            \\ \hline
% CT$\rightarrow$DD$\rightarrow$CR                  & 78.029                       & N*                            \\ \hline
% DD$\rightarrow$CT$\rightarrow$CD$\rightarrow$CR & 77.936                       & N*                            \\ \hline
% DD$\rightarrow$CD$\rightarrow$CT$\rightarrow$CR & 77.279                       & N*                            \\ \hline
% CT$\rightarrow$DD$\rightarrow$CD$\rightarrow$CR & 78.120                       & N*                            \\ \hline
% CT$\rightarrow$CD$\rightarrow$DD$\rightarrow$CR & 78.076                       & N*                            \\ \hline
% CD$\rightarrow$DD$\rightarrow$CT$\rightarrow$CR & 77.745                       & N*                            \\ \hline
% CD$\rightarrow$CT$\rightarrow$DD$\rightarrow$CR & 77.770                       & N*                            \\ \hline
% \end{tabular}%
% }
% \end{table}



% \begin{table}[]
% \centering
% \caption{The Performances of Fine-tuning Chain Models and Baselines whose Target Tasks are CD)}
% \label{tab:chain-performancescd}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Chain Models}                           & \textbf{Average MAP@R Scores} & \textbf{Positive Transfer?} \\ \hline
% CD                                                    & 0.869                                       & /                                     \\ \hline
% CT$\rightarrow$CR$\rightarrow$CD                  & 0.847                                       & N*                                    \\ \hline
% CT$\rightarrow$CD                                   & 0.871                                       & Y                                     \\ \hline
% CR$\rightarrow$CT$\rightarrow$CD                  & 0.862                                       & N                                     \\ \hline
% CR$\rightarrow$CD                                   & 0.853                                       & N*                                    \\ \hline
% DD$\rightarrow$CR$\rightarrow$CD                  & 0.855                                       & N*                                    \\ \hline
% DD$\rightarrow$CD                                   & 0.853                                       & N*                                    \\ \hline
% CR$\rightarrow$DD$\rightarrow$CD                  & 0.854                                       & N*                                    \\ \hline
% DD$\rightarrow$CT$\rightarrow$CD                  & 0.855                                       & N*                                    \\ \hline
% CT$\rightarrow$DD$\rightarrow$CD                  & 0.866                                       & N*                                    \\ \hline
% DD$\rightarrow$CT$\rightarrow$CR$\rightarrow$CD & 0.844                                       & N*                                    \\ \hline
% DD$\rightarrow$CR$\rightarrow$CT$\rightarrow$CD & 0.853                                       & N*                                    \\ \hline
% CT$\rightarrow$DD$\rightarrow$CR$\rightarrow$CD & 0.841                                       & N*                                    \\ \hline
% CT$\rightarrow$CR$\rightarrow$DD$\rightarrow$CD & 0.854                                       & N*                                    \\ \hline
% CR$\rightarrow$DD$\rightarrow$CT$\rightarrow$CD & 0.857                                       & N*                                    \\ \hline
% CR$\rightarrow$CT$\rightarrow$DD$\rightarrow$CD & 0.856                                       & N*                                    \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{table}[]
% \centering
% \caption{The Performances of Fine-tuning Chain Models and Baselines whose Target Tasks are DD)}
% \label{tab:chain-performancesdd}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Chain Models}                           & \textbf{Average Accuracies} & \textbf{Positive Transfer?} \\ \hline
% DD                                                    & 0.630                                          & /                                     \\ \hline
% CR$\rightarrow$DD                                   & 0.626                                          & N                                     \\ \hline
% CR$\rightarrow$CD$\rightarrow$DD                  & 0.610                                          & N*                                    \\ \hline
% CD$\rightarrow$DD                                   & 0.619                                          & N*                                    \\ \hline
% CD$\rightarrow$CR$\rightarrow$DD                  & 0.626                                          & N                                     \\ \hline
% CT$\rightarrow$DD                                   & 0.628                                          & N                                     \\ \hline
% CT$\rightarrow$CD$\rightarrow$DD                  & 0.610                                          & N*                                    \\ \hline
% CD$\rightarrow$CT$\rightarrow$DD                  & 0.628                                          & N                                     \\ \hline
% CT$\rightarrow$CR$\rightarrow$DD                  & 0.621                                          & N                                     \\ \hline
% CR$\rightarrow$CT$\rightarrow$DD                  & 0.627                                          & N                                     \\ \hline
% CT$\rightarrow$CR$\rightarrow$CD$\rightarrow$DD & 0.605                                          & N*                                    \\ \hline
% CT$\rightarrow$CD$\rightarrow$CR$\rightarrow$DD & 0.614                                          & N*                                    \\ \hline
% CR$\rightarrow$CT$\rightarrow$CD$\rightarrow$DD & 0.607                                          & N*                                    \\ \hline
% CR$\rightarrow$CD$\rightarrow$CT$\rightarrow$DD & 0.619                                          & N*                                    \\ \hline
% CD$\rightarrow$CT$\rightarrow$CR$\rightarrow$DD & 0.606                                          & N*                                    \\ \hline
% CD$\rightarrow$CR$\rightarrow$CT$\rightarrow$DD & 0.615                                          & N*                                    \\ \hline
% \end{tabular}%
% }
% \end{table}

\begin{table*}[]
\centering
\caption{The Performances of Fine-tuning Chain Models and Baselines (``+'' denotes positive transfer while ``-'' denotes negative transfer to the target tasks)}
\label{tab:chain-performances}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{|lc|lc|lc|lc|}
\hline
\multicolumn{2}{|c|}{\textbf{Code translation (CT)}} & \multicolumn{2}{c|}{\textbf{Code refinement (CR)}} & \multicolumn{2}{c|}{\textbf{Clone detection (CD)}} & \multicolumn{2}{c|}{\textbf{Defect defection (DD)}} \\ \hline
\multicolumn{1}{|c|}{Models} & \begin{tabular}[c]{@{}c@{}}Average \\ BLEU Scores\end{tabular} & \multicolumn{1}{c|}{Models} & \begin{tabular}[c]{@{}c@{}}Average \\ BLEU Scores\end{tabular} & \multicolumn{1}{c|}{Models} & \begin{tabular}[c]{@{}c@{}}Average \\ MAP@R Score\end{tabular} & \multicolumn{1}{c|}{Models} & \begin{tabular}[c]{@{}c@{}}Average\\ Accuracy\end{tabular} \\ \hline
\multicolumn{1}{|l|}{CT}              & 70.881                       & \multicolumn{1}{l|}{CR}              & 79.566                       & \multicolumn{1}{l|}{CD}              & 0.869                         & \multicolumn{1}{l|}{DD}              & 0.630                       \\ \hline
\multicolumn{1}{|l|}{CR$\rightarrow$CT}           & \textbf{74.242 (+)}          & \multicolumn{1}{l|}{CT$\rightarrow$CR}           & \textbf{76.824 (-)}          & \multicolumn{1}{l|}{CT$\rightarrow$CD}           & 0.871                         & \multicolumn{1}{l|}{CR$\rightarrow$DD}           & 0.626                       \\ \hline
\multicolumn{1}{|l|}{CD$\rightarrow$CT}           & 70.879                       & \multicolumn{1}{l|}{CD$\rightarrow$CR}           & 79.643                       & \multicolumn{1}{l|}{CR$\rightarrow$CD}           & \textbf{0.853 (-)}            & \multicolumn{1}{l|}{CD$\rightarrow$DD}           & \textbf{0.619 (-)}          \\ \hline
\multicolumn{1}{|l|}{DD$\rightarrow$CT}           & 70.839                       & \multicolumn{1}{l|}{DD$\rightarrow$CR}           & 79.712                       & \multicolumn{1}{l|}{DD$\rightarrow$CD}           & \textbf{0.853 (-)}            & \multicolumn{1}{l|}{CT$\rightarrow$DD}           & 0.628                       \\ \hline
\multicolumn{1}{|l|}{CR$\rightarrow$CD$\rightarrow$CT}        & \textbf{73.957 (+)}          & \multicolumn{1}{l|}{CT$\rightarrow$CD$\rightarrow$CR}        & \textbf{77.870 (-)}          & \multicolumn{1}{l|}{CT$\rightarrow$CR$\rightarrow$CD}        & \textbf{0.847 (-)}            & \multicolumn{1}{l|}{CR$\rightarrow$CD$\rightarrow$DD}        & \textbf{0.610 (-)}          \\ \hline
\multicolumn{1}{|l|}{CD$\rightarrow$CR$\rightarrow$CT}        & \textbf{75.058 (+)}          & \multicolumn{1}{l|}{CD$\rightarrow$CT$\rightarrow$CR}        & \textbf{77.455 (-)}          & \multicolumn{1}{l|}{CR$\rightarrow$CT$\rightarrow$CD}        & 0.862                         & \multicolumn{1}{l|}{CD$\rightarrow$CR$\rightarrow$DD}        & 0.626                       \\ \hline
\multicolumn{1}{|l|}{DD$\rightarrow$CD$\rightarrow$CT}        & 70.739                       & \multicolumn{1}{l|}{DD$\rightarrow$CD$\rightarrow$CR}        & 79.825                       & \multicolumn{1}{l|}{DD$\rightarrow$CR$\rightarrow$CD}        & \textbf{0.855 (-)}            & \multicolumn{1}{l|}{CT$\rightarrow$CD$\rightarrow$DD}        & \textbf{0.610 (-)}          \\ \hline
\multicolumn{1}{|l|}{CD$\rightarrow$DD$\rightarrow$CT}        & 71.000                       & \multicolumn{1}{l|}{CD$\rightarrow$DD$\rightarrow$CR}        & 79.616                       & \multicolumn{1}{l|}{CR$\rightarrow$DD$\rightarrow$CD}        & \textbf{0.854 (-)}            & \multicolumn{1}{l|}{CD$\rightarrow$CT$\rightarrow$DD}        & 0.628                       \\ \hline
\multicolumn{1}{|l|}{DD$\rightarrow$CR$\rightarrow$CT}        & \textbf{74.113 (+)}          & \multicolumn{1}{l|}{DD$\rightarrow$CT$\rightarrow$CR}        & \textbf{77.347 (-)}          & \multicolumn{1}{l|}{DD$\rightarrow$CT$\rightarrow$CD}        & \textbf{0.855 (-)}            & \multicolumn{1}{l|}{CT$\rightarrow$CR$\rightarrow$DD}        & 0.621                       \\ \hline
\multicolumn{1}{|l|}{CR$\rightarrow$DD$\rightarrow$CT}        & \textbf{74.118 (+)}          & \multicolumn{1}{l|}{CT$\rightarrow$DD$\rightarrow$CR}        & \textbf{78.029 (-)}          & \multicolumn{1}{l|}{CT$\rightarrow$DD$\rightarrow$CD}        & \textbf{0.866 (-)}            & \multicolumn{1}{l|}{CR$\rightarrow$CT$\rightarrow$DD}        & 0.627                       \\ \hline
\multicolumn{1}{|l|}{DD$\rightarrow$CR$\rightarrow$CD$\rightarrow$CT}     & \textbf{73.942 (+)}          & \multicolumn{1}{l|}{DD$\rightarrow$CT$\rightarrow$CD$\rightarrow$CR}     & \textbf{77.936 (-)}          & \multicolumn{1}{l|}{DD$\rightarrow$CT$\rightarrow$CR$\rightarrow$CD}     & \textbf{0.844 (-)}            & \multicolumn{1}{l|}{CT$\rightarrow$CR$\rightarrow$CD$\rightarrow$DD}     & \textbf{0.605 (-)}          \\ \hline
\multicolumn{1}{|l|}{DD$\rightarrow$CD$\rightarrow$CR$\rightarrow$CT}     & \textbf{73.950 (+)}          & \multicolumn{1}{l|}{DD$\rightarrow$CD$\rightarrow$CT$\rightarrow$CR}     & \textbf{77.279 (-)}          & \multicolumn{1}{l|}{DD$\rightarrow$CR$\rightarrow$CT$\rightarrow$CD}     & \textbf{0.853 (-)}            & \multicolumn{1}{l|}{CT$\rightarrow$CD$\rightarrow$CR$\rightarrow$DD}     & \textbf{0.614 (-)}          \\ \hline
\multicolumn{1}{|l|}{CR$\rightarrow$DD$\rightarrow$CD$\rightarrow$CT}     & \textbf{74.145 (+)}          & \multicolumn{1}{l|}{CT$\rightarrow$DD$\rightarrow$CD$\rightarrow$CR}     & \textbf{78.120 (-)}          & \multicolumn{1}{l|}{CT$\rightarrow$DD$\rightarrow$CR$\rightarrow$CD}     & \textbf{0.841 (-)}            & \multicolumn{1}{l|}{CR$\rightarrow$CT$\rightarrow$CD$\rightarrow$DD}     & \textbf{0.607 (-)}          \\ \hline
\multicolumn{1}{|l|}{CR$\rightarrow$CD$\rightarrow$DD$\rightarrow$CT}     & \textbf{73.882 (+)}          & \multicolumn{1}{l|}{CT$\rightarrow$CD$\rightarrow$DD$\rightarrow$CR}     & \textbf{78.076 (-)}          & \multicolumn{1}{l|}{CT$\rightarrow$CR$\rightarrow$DD$\rightarrow$CD}     & \textbf{0.854 (-)}            & \multicolumn{1}{l|}{CR$\rightarrow$CD$\rightarrow$CT$\rightarrow$DD}     & \textbf{0.619 (-)}          \\ \hline
\multicolumn{1}{|l|}{CD$\rightarrow$DD$\rightarrow$CR$\rightarrow$CT}     & \textbf{74.606 (+)}          & \multicolumn{1}{l|}{CD$\rightarrow$DD$\rightarrow$CT$\rightarrow$CR}     & \textbf{77.745 (-)}          & \multicolumn{1}{l|}{CR$\rightarrow$DD$\rightarrow$CT$\rightarrow$CD}     & \textbf{0.857 (-)}            & \multicolumn{1}{l|}{CD$\rightarrow$CT$\rightarrow$CR$\rightarrow$DD}     & \textbf{0.606 (-)}          \\ \hline
\multicolumn{1}{|l|}{CD$\rightarrow$CR$\rightarrow$DD$\rightarrow$CT}     & \textbf{74.204 (+)}          & \multicolumn{1}{l|}{CD$\rightarrow$CT$\rightarrow$DD$\rightarrow$CR}     & \textbf{77.770 (-)}          & \multicolumn{1}{l|}{CR$\rightarrow$CT$\rightarrow$DD$\rightarrow$CD}     & \textbf{0.856 (-)}            & \multicolumn{1}{l|}{CD$\rightarrow$CR$\rightarrow$CT$\rightarrow$DD}     & \textbf{0.615 (-)}          \\ \hline
\end{tabular}%
}
\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[ht]
% \centering
% \caption{The Performances of Fine-tuning Chains whose Target Task is CR}
% \label{tab:CR-performances}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Fine-tuning Chains}                           & \textbf{Average BLEU Scores} & \textbf{Successful Transfer?} \\ \hline
% CR                                                    & 79.566                       & /                             \\ \hline
% CT$\rightarrow$CR                                   & 76.824                       & N*                            \\ \hline
% CT$\rightarrow$CD$\rightarrow$CR                  & 77.870                       & N*                            \\ \hline
% CD$\rightarrow$CT$\rightarrow$CR                  & 77.455                       & N*                            \\ \hline
% CD$\rightarrow$CR                                   & 79.643                       & Y                             \\ \hline
% DD$\rightarrow$CR                                   & 79.712                       & Y                             \\ \hline
% DD$\rightarrow$CD$\rightarrow$CR                  & 79.825                       & Y                             \\ \hline
% CD$\rightarrow$DD$\rightarrow$CR                  & 79.616                       & Y                             \\ \hline
% DD$\rightarrow$CT$\rightarrow$CR                  & 77.347                       & N*                            \\ \hline
% CT$\rightarrow$DD$\rightarrow$CR                  & 78.029                       & N*                            \\ \hline
% DD$\rightarrow$CT$\rightarrow$CD$\rightarrow$CR & 77.936                       & N*                            \\ \hline
% DD$\rightarrow$CD$\rightarrow$CT$\rightarrow$CR & 77.279                       & N*                            \\ \hline
% CT$\rightarrow$DD$\rightarrow$CD$\rightarrow$CR & 78.120                       & N*                            \\ \hline
% CT$\rightarrow$CD$\rightarrow$DD$\rightarrow$CR & 78.076                       & N*                            \\ \hline
% CD$\rightarrow$DD$\rightarrow$CT$\rightarrow$CR & 77.745                       & N*                            \\ \hline
% CD$\rightarrow$CT$\rightarrow$DD$\rightarrow$CR & 77.770                       & N*                            \\ \hline
% \end{tabular}%
% }
% \end{table}


% \begin{center}
%     \begin{tabular}{| l | l | l |}
%     \hline    
%     \multicolumn{3}{|c|}{CR Table} \\
%     \hline
%     \textbf{Task\_Path}      &   \textbf{Avg\_Score(Bleu Score)}               &       \textbf{Is\_Better?} \\
%     \hline
%     CR              &       79.566                              &       /  \\
%     \hline
%     CT->CR          &       76.824                              &       N* \\
%     \hline
%     CT->CD->CR      &       77.870                              &       N* \\
%     \hline
%     CD->CT->CR      &       77.455                              &       N* \\
%     \hline
%     CD->CR          &       79.643                              &       Y  \\
%     \hline
%     DD->CR          &       79.712                              &       Y  \\
%     \hline
%     DD->CD->CR      &       79.825                              &       Y  \\
%     \hline
%     CD->DD->CR      &       79.616                              &       Y  \\
%     \hline
%     DD->CT->CR      &       77.347                              &       N* \\
%     \hline
%     CT->DD->CR      &       78.029                              &       N* \\
%     \hline
%     DD->CT->CD->CR  &       77.936                              &       N* \\
%     \hline
%     DD->CD->CT->CR  &       77.279                              &       N* \\
%     \hline
%     CT->DD->CD->CR  &       78.120                              &       N* \\
%     \hline
%     CT->CD->DD->CR  &       78.076                              &       N* \\
%     \hline
%     CD->DD->CT->CR  &       77.745                              &       N* \\
%     \hline
%     CD->CT->DD->CR  &       77.770                              &       N* \\
%     \hline
%     \end{tabular}
% \end{center}




==> figures/05-discussion.tex <==
\section{Analyses of Explanatory Factors}
\label{sec:discussion}

To determine the factors that may help explain the positive and negative transfer patterns we found, we conducted multiple analyses from three perspectives: dataset, task, and model (as shown in Figure 2). For \textbf{Pattern 1} and \textbf{Pattern 2}, the intermediate tasks fine-tuned in between do not affect the statistical significance of negative transfer/positive transfer. %For \textbf{Pattern 2}, the intermediate tasks fine-tuned before CD do not affect the statistical significance as long as CD is \textit{immediately} fine-tuned before DD.% 
Based on these findings, we simplify our analyses by only focusing on CR$\rightarrow$CT, CT$\rightarrow$CR %CD$\rightarrow$DD% 
fine-tuning chain models. In this section, we report the results of each analysis and provide possible explanations based on the results.

% \subsection{Data: Domain Similarity}

% \hl{in the table instead of only putting i an ii, add word such as truncate and split also update method with same words so that people can refer back}

% \hl{this table should be a single column table not a full column}
% Table \ref{tab:textemb} shows the cosine similarities between the TEXTEMBs of every two task-specific datasets calculated in the two ways we introduced in Section \ref{sec:method} (i.e. \textbf{\textit{Truncation}} and \textbf{\textit{Split}})\hl{????}. The similarity between any two datasets is relatively low with the highest cosine similarity of around 0.08, which suggests that code and domain properties of any two datasets captured by the pre-trained CodeBERT model are not similar to each other. 
% \hl{reduce Vu's findings to 1 sentence. or even better say our findings and simply says "which matches to Vu et al.'s findings"}

% %Vu et al.~\cite{vu2020exploring} conducted experiments with NLP tasks to rank all other tasks as intermediate tasks in descending order by cosine similarity between their TEXTEMBs and target task's TEXTEMB, given a specific target task. The goal was to select the best intermediate task for a given target task based on the ranking. However, they found that TEXTEMB performed badly for text classification/regression NLP tasks whose datasets are relatively homogeneous than other NLP tasks. The authors argued that TEXTEMB might have trouble predicting successful transfer between tasks when domain similarity captured by it is not an effective or relevant transfer factor. 

% According to our Table \ref{tab:textemb}, there is not a clear way of identifying the positive transfer task orderings by simply looking at the cosine similarities, which matches Vu et al.'s~\cite{vu2020exploring} findings. Therefore, we believe that TEXTEMB offers no explanatory power to explaining our discovered task ordering patterns. 


% \begin{mdframed}[roundcorner=10pt]
% \textbf{Finding 1: Dataset domain similarity measured by TEXTEMB offers no explanatory power to explaining our discovered task ordering patterns} 
% \end{mdframed}

% \hl{mute findings that don't show any significant result}

% \begin{table}[ht]
% \caption{TEXTEMB Cosine Similarity between Datasets}
% \label{tab:textemb}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
%                                                                                                    & \textbf{CD VS DD} & \textbf{CD VS CR} & \textbf{CD VS CT} & \textbf{DD VS CR} & \textbf{DD VS CT} & \textbf{CR VS CT} \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Cosine Similarity of \\ TEXTEMB for approach (i)\end{tabular}}  & 0.02001           & 0.07765           & 0.04007           & 0.07130           & 0.02727           & 0.02903           \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Cosine Similarity of \\ TEXTEMB for approach (ii)\end{tabular}} & 0.01063           & 0.06467           & 0.02300           & 0.08021           & 0.03228           & 0.02938           \\ \hline
% \end{tabular}%
% }
% \end{table}
\subsection{Data: Syntactical Similarity Analysis}
In this section, we provide the average similarity scores for the dataset pairs (CR and CT) and (CD and DD) across keywords, operators, and identifiers. Although the two patterns we discovered are CR$\rightarrow$CT, and CT$\rightarrow$CR, we report the results of both (CR and CT) datasets and (CD and DD) datasets because we want to have a reference point for comparison. Our results demonstrate that the CR and CT datasets have a higher similarity in terms of operators (0.342 for 12,676,329 pairs of code snippets in CR and CT compared to 0.295 for 12,836,220 pairs of code snippets in CD and DD). However, they exhibit lower similarity in terms of keywords (0.247 for 13,789,146 pairs of code snippets in CR and CT compared to 0.305 for 12,850,932 pairs of code snippets in CD and DD) and identifiers (0.006 for 13,789,146 pairs of code snippets in CR and CT compared to 0.025 for 12,858,288 pairs of code snippets in CD and DD).

The lower similarity in keywords and identifiers between the CR and CT datasets compared to the CD and DD datasets may be explained by the difference in programming languages used. Specifically, the former uses Java and C\#, while the latter uses C/C++. Since Java and C\# have distinct keywords whereas C and C++ have similar keywords, this difference in programming languages could explain the lower similarity in terms of keywords. Furthermore, our findings regarding identifiers do not correspond with the findings in ~\cite{ahmed2022multilingual}. We speculate that the differences in our findings regarding identifiers compared to ~\cite{ahmed2022multilingual} is likely due to the disparities in the datasets used. The study by ~\cite{ahmed2022multilingual} utilized the ROSETTACODE dataset~\cite{RosettaCodeData} which consists of a large number of problems. For each problem, the answer is provided by code snippets written in different languages, which makes their meanings semantically equivalent. In contrast, our datasets do not have access to code snippets with similar semantic meanings, which could be the reason for the differences in our conclusions regarding identifiers. As a conclusion, we suggest that the higher similarity in terms of operators used in CR and CT could potentially account for the positive transfer (\textbf{Pattern 1}), as discussed in Section \ref{sec:results}.

%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 1: The shared operators within the CR and CT datasets could be a possible explanation.
%} 
%\end{mdframed}

\observation{The shared operators within the CR and CT datasets could be a possible explanation.}


\subsection{Data: Semantic Similarity Analysis}

% Since our study revealed that CD$\rightarrow$DD and CT$\rightarrow$CR are negative transfer patterns (\textbf{Pattern 2 \& 3}), while CR improves CT's performance, we will concentrate on analyzing the (CR, CT) and (CD, DD) dataset pairs in this symmetrical examination.

We present our results of semantic similarity analysis for task pairs (CD, DD) and (CR, CT) in this section. Although the two patterns we discovered are CR$\rightarrow$CT, and CT$\rightarrow$CR, we report the results of both (CR and CT) datasets and (CD and DD) datasets because we want to have a reference point for comparison purpose. We report our semantic similarity for each pair of datasets by using the average cosine similarity scores of all pairs of code snippets in that pair of datasets. Our results show that the average similarity score for CD and DD's training datasets is 0.317 for a total of 421,838 pairs of code snippets, whereas the average similarity score for CR and CT's training datasets is 0.410 for a total of 1,645,128 pairs of code snippets. Based on these results, we could see that the code snippets in CR are more semantically similar to those in CT datasets than code snippets in CD dataset to DD datasets. This result indicates that the semantic similarity of code snippets between training datasets of different tasks could be a relevant factor to consider when selecting multiple SE tasks as intermediate tasks to enhance model performance. 

% Our analyses indicates that the average closeness of the top 10 results for CD and DD's training datasets is 0.57011, whereas the average closeness of the top 10 results for CR and CT's training datasets is 0.706529.



%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 2: Choosing datasets that are more semantically similar could lead to better performance.} 
%\end{mdframed}

\observation{Choosing datasets that are more semantically similar could lead to better performance.}

% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[]
% \centering
% \caption{Semantic Analysis  Top 10 Results Table}
% \label{tab:cosinecom-results}
% \begin{tabular}{|l|l|}
% \hline
% \textbf{CD and DD} & \textbf{CR and CT} \\ \hline
% 0.57942 & 0.73186 \\ \hline
% 0.57876 & 0.71808 \\ \hline
% 0.57307 & 0.71702 \\ \hline
% 0.57042 & 0.71448 \\ \hline
% 0.57033 & 0.71011 \\ \hline
% 0.57004 & 0.70479 \\ \hline
% 0.56585 & 0.69435 \\ \hline
% 0.56456 & 0.69273 \\ \hline
% 0.56444 & 0.69202 \\ \hline
% 0.56426 & 0.68985 \\ \hline
% \end{tabular}
% \end{table}



%\begin{table}[ht]
%\centering
%\caption{Semantic Analysis  Top 10 Results Table}
%\label{tab:cosinecom-results}
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{|l|l|}
%\hline
%\textbf{CD and DD} & \textbf{CR and CT}           \\ \hline
%0.57942            & 0.73186                      \\ \hline
%0.57876            & 0.71808                      \\ \hline
%0.57307            & 0.71702                      \\ \hline
%0.57042            & 0.71448                      \\ \hline
%0.57033            & 0.71011                      \\ \hline
%0.57004            & 0.70479                      \\ \hline
%0.56585            & 0.69435                      \\ \hline
%0.56456            & 0.69273                      \\ \hline
%0.56444            & 0.69202                      \\ \hline
%0.56426            & 0.68985                      \\ \hline
%\end{tabular}%
%}
%\end{table}



% \begin{table}[ht]
% \centering
% \caption{Common Program Representation Cosine Similarity between CD and DD Datasets}
% \label{tab:cosinecom-cddd}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Data Index} & \textbf{Data Index} & \textbf{Cosine Similarity} \\ \hline
% 18448               & 4562                & 0.57942                    \\ \hline
% 18448               & 13528               & 0.57876                    \\ \hline
% 15362               & 15745               & 0.57307                    \\ \hline
% 18448               & 2266                & 0.57042                    \\ \hline
% 15362               & 9879                & 0.57033                    \\ \hline
% 10961               & 13528               & 0.57004                    \\ \hline
% 1289                & 13528               & 0.56585                    \\ \hline
% 20181               & 6652                & 0.56456                    \\ \hline
% 15362               & 2638                & 0.56444                    \\ \hline
% 1617                & 5                   & 0.56426                    \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{center}
%     \begin{tabular}{|l | l |l|}
%     \hline    
%     \multicolumn{3}{|c|}{\textbf{CD\_POJ104\_DD\_DEVIGN Table}} \\
%     \hline
%     Data\_Index   &    Data\_Index   &   Closeness     \\
%     \hline
%     18448     &       4562   &   0.57942   \\
%     \hline
%     18448     &       13528  &   0.57876   \\
%     \hline
%     15362     &       15745  &   0.57307   \\
%     \hline
%     18448     &       2266   &   0.57042   \\
%     \hline
%     15362     &       9879   &   0.57033   \\
%     \hline
%     10961     &       13528  &   0.57004   \\
%     \hline
%     1289      &       13528  &   0.56585   \\
%     \hline
%     20181     &       6652   &   0.56456   \\
%     \hline
%     15362     &       2638   &   0.56444   \\
%     \hline
%     1617      &       5      &   0.56426   \\
%     \hline
%     \end{tabular}
% \end{center}

% \begin{table}[ht]
% \centering
% \caption{Common Program Representation Cosine Similarity between CR and CT Datasets}
% \label{tab:ctcrcom}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Data Index} & \textbf{Data Index} & \textbf{Cosine Similarity} \\ \hline
% 23651               & 2755                & 0.73186                    \\ \hline
% 31724               & 2755                & 0.71808                    \\ \hline
% 42120               & 8213                & 0.71702                    \\ \hline
% 42120               & 3486                & 0.71448                    \\ \hline
% 42120               & 5521                & 0.71011                    \\ \hline
% 33581               & 7541                & 0.70479                    \\ \hline
% 2079                & 1139                & 0.69435                    \\ \hline
% 23651               & 4077                & 0.69273                    \\ \hline
% 28015               & 6393                & 0.69202                    \\ \hline
% 32338               & 4243                & 0.68985                    \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{center}
%     \begin{tabular}{| l | l | l |}
%     \hline    
%     \multicolumn{3}{|c|}{\textbf{CR\_BUGS2FIX\_CT\_CODETRANS Table}} \\
%     \hline
%     Data\_Index   &    Data\_Index   &   Closeness     \\
%     \hline
%     23651     &       2755  &   0.73186   \\
%     \hline
%     31724     &       2755  &   0.71808   \\
%     \hline
%     42120     &       8213  &   0.71702   \\
%     \hline
%     42120     &       3486  &   0.71448   \\
%     \hline
%     42120     &       5521  &   0.71011   \\
%     \hline
%     33581     &       7541  &   0.70479   \\
%     \hline
%     2079      &       1139  &   0.69435   \\
%     \hline
%     23651     &       4077  &   0.69273   \\
%     \hline
%     28015     &       6393  &   0.69202   \\
%     \hline
%     32338     &       4243  &   0.68985   \\

%     \hline
%     \end{tabular}
% \end{center}


% \subsection{Data: Covariance Matrix Analysis}
% In light of the patterns we identified in Section \ref{sec:results}, we analyze the four tasks in two pairs, CR-CT and CD-DD. Our findings from the covariance matrix analysis are presented in Table \ref{tab:covarmatrix}. The distance is calculated using the Frobenius Norm~\cite{herdin2005correlation}, which captures the alignment of data points between two datasets.

% \hl{the text in first 2 coulmns of table 7 is cryptic! what does it mean?}
% According to Wu et al.~\cite{wu2020understanding}, the alignment of two datasets is an indicator of the quality of the knowledge transfer between them. This means that a smaller distance between the covariance matrices indicates more positive knowledge transfer. However, our results show the opposite, with the CT-CR dataset pair being more distant from each other than the CD-DD pair. We attribute this to the differences in the training method between ours and the multi-task learning approach~\cite{ruder2017overview}. Specifically, our method only has a shared module and does not include task-specific modules. Additionally, we train one task at a time, while multi-task learning trains multiple tasks together. We believe that these differences in training method contribute to the opposite observation of CR-CT and CD-DD. In our method, the later task dominates the weight, while in multi-task learning, the weights are updated based on all tasks and the contribution of each task to the total loss is determined by the weight used for each individual loss. \hl{so why would this result in a higher score for CR-CT?}

% Furthermore, it is worth noting that the multi-task learning approach employs a loss function that sums the losses of all tasks involved, with adjustable weights. This loss function can be expressed as L = $\sum_{i=1}^{n}${$w_{i}$*$L_i$}, where n denotes the total number of tasks and $L_i$ represents the loss function for task i. The impact of each task on the updates of shared weights is variable because of the adjustable weights. \hl{why do I need to know this?}

% \hl{I am not buying this explanation}

% \begin{mdframed}[roundcorner=10pt]
% \textbf{Finding 3: The reason for the discrepancy between ours and the findings from ~\cite{wu2020understanding} is that, despite CT and CR exhibiting worse data alignment than CD and DD, the CR$\rightarrow$CT chain performs better than CD$\rightarrow$DD due to differences in the weight updating method.} 
% \end{mdframed}

% \hl{Not buying the Findings}

% \begin{table}[ht]
% \centering
% \caption{Covariance Matrix Distance Result}
% \label{tab:covarmatrix}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Task-specific Dataset} & \textbf{Task-specific Dataset} & \textbf{Distance} \\ \hline
% CT\_CODETRANS\_Input           & CR\_BUGS2FIX\_Output           & 0.78057           \\ \hline
% CR\_BUGS2FIX\_Input            & CT\_CODETRANS\_Input           & 0.78053           \\ \hline
% CR\_BUGS2FIX\_Output           & CT\_CODETRANS\_Output          & 0.78050           \\ \hline
% CR\_BUGS2FIX\_Input            & CT\_CODETRANS\_Output          & 0.78046           \\ \hline
% CD\_POJ104                     & DD\_DEVIGN                     & 0.31759           \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{center}
%     \begin{tabular}{| l | l | l|}
%     \hline    
%     \multicolumn{3}{|c|}{\textbf{Covariance Matrix Distance Result Table}} \\
%     \hline
%     Dataset1                    &    Dataset2                   &   Distance  \\
%     \hline
%     CT\_CODETRANS\_Input        &       CR\_BUGS2FIX\_Output    &   0.78057   \\
%     \hline
%     CR\_BUGS2FIX\_Input         &       CT\_CODETRANS\_Input    &   0.78053   \\
%     \hline
%     CR\_BUGS2FIX\_Output        &       CT\_CODETRANS\_Output   &   0.78050   \\
%     \hline
%     CR\_BUGS2FIX\_Input         &       CT\_CODETRANS\_Output   &   0.78046   \\
%     \hline
%     CD\_POJ104                  &       DD\_DEVIGN              &   0.31759   \\
%     \hline
%     \end{tabular}
% \end{center}




% \begin{table}[ht]
% \caption{Keywords, Operators, and Identifier Similarity}
% \label{tab:syntaxsim}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|}
% \hline
% \textbf{Dataset Pair} & \textbf{Operators} & \textbf{Keywords} & \textbf{Identifiers} \\ \hline
% (CR, CT)              & 0.34188            & 0.24677           & 0.005942             \\ \hline
% (CD, DD)              & 0.29498            & 0.30437           & 0.024607             \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{center}
%     \begin{tabular}{| l | l | l | l |}
%     \hline    
%     \multicolumn{4}{|c|}{\textbf{Keywords Operators Identifiers Similarities}} \\
%     \hline
%     Dataset Pair    &   Operators    &   Keywords    &   Identifiers     \\
%     \hline
%     CR, CT          &   0.34188                 &   0.24677                &    0.005942\\
%     \hline
%     CD, DD          &   0.29498                 &   0.30437                &    0.024607\\
%     \hline
%     \end{tabular}
% \end{center}


\subsection{Data: Dataset Size Impact Analysis}
%Since we posit that the size of the fine-tuning dataset might play an important role in the transferability between intermediate SE task and target task of interest, it might help to explain the cause of those interesting fine-tuning chain patterns we identified. In this experiment, we only focus on the fine-tuning chain patterns that we found in Section \ref{sec:results}. To make the fine-tuning process with four data regimes (\textit{FULL to FULL}, \textit{LIMITED to FULL}, \textit{LIMITED to LIMITED}, and \textit{FULL to LIMITED}) manageable and provide a deeper analysis on the three fine-tuning chain patterns, we only conduct fine-tuning for chains of two tasks with all four data regimes using 10-fold cross validation. For example, to perform dataset size analysis on \textbf{Pattern 1}, the four data regimes of source-target pairs would be applied to CR-CT (i.e. first fine-tune the model with CR then fine-tune CT where CT is the target task and CR is the intermediate/source task.) The models fine-tuned in \textit{FULL to FULL} and \textit{LIMITED to FULL} data regimes would still be compared with \textit{FULL} baselines created in Section \ref{}, while the \textit{LIMITED to LIMITED} and \textit{FULL to LIMITED} ones are compared with \textit{LIMITED} baselines. The results of the comparisons are then tested by Welch's t-test for the statistical significance.

%We show the results of dataset size analysis in Table X. For \textbf{Pattern 1} where CT's performance is boosted by CR as an intermediate task, the increasing dataset size of CR leads to a larger performance boost of CT. For \textbf{Pattern 2}, the general trend is the increasing dataset size of CD caused DD to go from a performance boost to a performance drop compared to its baseline, indicating that increasing dataset size of CD has a detrimental effect on DD's performance (While the performance difference in terms of 10-fold cross validation between DD's \textit{LIMITED} baseline and \textit{FULL to LIMITED}/\textit{LIMITED to LIMITED} is not statistically significant, the general trend still holds). Finally, CT hurts the performance of CR (\textbf{Pattern 3}). The performance difference between CR's \textit{FULL} baseline and CT-CR's \textit{LIMITED to FULL} fine-tuned model was not statistically significant (only 0.23 average BLEU score difference). When the data regime of CT-CR changed to \textit{FULL to FULL}, the performance difference became statistically significant with a 2.742 average BLEU score difference, which means that the decreasing dataset size of CT mitigates the performance drop for CR. However, when the data regime changed from \textit{LIMITED to LIMITED} to \textit{FULL to LIMITED}, CT actually boosted CR's performance even more, which is against our \textbf{Pattern 3}. We posit that other factors might have contributed to \textbf{Pattern 3} where dataset size alone may not be enough. 

Among all task-specific datasets, CT's task-specific dataset has the smallest number of samples (Table \ref{tab:tasks}). When CT is designated as the target task, its performance improves by intermediate task fine-tuning in most of the fine-tuning chain models. And it is the only task that shows positive transfer by intermediate task fine-tuning in our experiments. This observation aligns with the argument in NLP literature that target tasks with smaller datasets benefit the most from intermediate task fine-tuning~\cite{vu2020exploring, pruksachatkun2020intermediate, chang2021rethinking}. Since CT is the task whose training dataset has the smallest amount of samples among all four SE tasks, we believe the dataset size plays a role in explaining its boosted performance after fine-tuning other tasks (\textbf{Pattern 1}), especially CR. However, we should note that CT's performance is not always boosted by all intermediate tasks: when CR is not one of the intermediate tasks, CT's performance remains almost unchanged.

Regarding intermediate tasks, CR's dataset has the largest number of samples. Yet, it only enhances CT's performance instead of other tasks (\textbf{Pattern 1}). These findings resemble those in NLP literature, which suggest that intermediate task data size does not have consistent effect on target task performance
~\cite{pruksachatkun2020intermediate}. For \textbf{Pattern 2}, CT does not improve any other target tasks' performances. However,  Vu et al.~\cite{vu2020exploring} argued that positive transfer is still possible even when the intermediate task dataset is small. Since we do not have any other tasks whose training data is relatively the same size as CT's, it is not reasonble to draw any conclusions for this pattern. Consequently, dataset size may not adequately explain the underlying reasons for the two task ordering patterns (\textbf{Pattern 1 \& 2}) we identified.
%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 3: Task-specific dataset size can not sufficiently explain both positive and negative transfer task ordering patterns.} 
%\end{mdframed}

\textcolor{blue}{DRAFT-Jiawei: To get a fine-grained analysis on the explanation of Pattern 1 \& 2 in terms of dataset size, we conducted an experiment where we controlled the dataset sizes of the intermediate task and target task. Similar to what Vu et al. ~\cite{vu2020exploring} did, we performed transfer experiments in four data regimes to examine the impact of dataset size on intermediate-to-target task transfer (i.e. Pattern 1 \& 2): FULL $\rightarrow$ FULL, FULL $\rightarrow$ LIMITED, LIMITED $\rightarrow$ FULL, LIMITED $\rightarrow$ LIMITED. In the FULL training regime, all training data for the associated task is used for fine-tuning. In the LIMITED regime, we randomly sampled 1K training data instances without replacement. The models that were only fine-tuned with target tasks' datasets (FULL/LIMITED) without any intermediate fine-tuning were set as baselines. Since we trained the models with 10-fold cross validation, we conducted Welch's t-test ~\cite{} to measure the statistical significance of the performance difference between fine-tuning chain models and baselines trained with different data regimes to identify the performance boost or drop. The experiment results for Pattern 1 and 2 are shown in Table \ref{}. For Pattern 1, increasing the amount of intermediate task's training data continued to boost the performances of both FULL and LIMITED baselines further. For CT's LIMITED baseline, its performance got boosted more significantly than CT's FULL baseline (49.998-24.841 VS 74.242 -70.881). This may indicate that increasing the dataset size for intermediate task can help the target task with scarce data availablility. For Pattern 2, the performance drops for FULL baseline when CT was the intermediate task before CR. However, for LIMITED baseline, the performance increased when CT was fine-tuning before CR. Since CR has the largest trainined dataset, we posit that only using LIMITED data regime was not enough that might have led to underfit of the model. When CR is fully trained with FULL data regime, fine-tuning CT before it as an intermediate task decreases its performance. With more data of CT, the performance drops more. Therefore, we believe...}

\observation{Task-specific dataset size can not sufficiently explain both positive and negative transfer task ordering patterns.}


\subsection{Task: Affinity}
We present the results of task affinity analysis for the task orderings CR$\rightarrow$CT, and CT$\rightarrow$CR in the Table \ref{tab:task-affinity}. In addition, we include the affinity scores for the CT, and CR baseline models for comparison purposes. Note that the affinity score for a model is calculated as the sum of the loss differences between that model and the baseline model over 100 steps. 

\textit{Explanation for \textbf{Pattern 1}:}
Given the target task of CT, the intermediate fine-tuned model is the resulting model after training the pre-trained model with CR task (CR baseline in this case). The affinity score for the intermediate fine-tuned model is -6.121, while the pre-trained model has an affinity score of -6.987. The affinity score for the intermediate fine-tuned model is larger than the affinity score for the pre-trained model. This suggests that there is a low task affinity value between CR and CT because the intermediate fine-tuned model is further away from the baseline model compared to the pre-trained model. This result suggests that the training on CR has a small negative impact on the performance of the subsequent CT task. This is contradicted to the positive transfer we observed for the CR$\rightarrow$CT.

% \hl{why do we speculate this? what is the possible rationale? I don't think it's intuitive, actually I don't even know why would less steps result into this? Needs explanation instead of just saying a statement and hoping that reader will be able to figure it out}
% % \hl{i thought }
% \noindent\textit{Affinity score for \textbf{Pattern 2 (CD$\rightarrow$DD)}:}
% Given the target task of DD, The intermediate fine-tuned model is the resulting model after training CD on the pre-trained model (CD baseline in this case). The affinity score for the intermediate fine-tuned model is -0.241, while the pre-train model has an affinity score of -0.2586. The affinity score for intermediate fine-tuned model is found to be similar to that of the pre-trained model, indicating that there is low affinity between CD and DD. Despite observing a significant decrease in the performance of the CD$\rightarrow$DD task ordering, this is not clearly reflected in the affinity score. Similarly, we posit that this might be caused by the small number of steps used in the study. \hl{same comment as before}

\textit{Explanation for \textbf{Pattern 2}:}
Given the target task of CR, The intermediate fine-tuned model is the resulting model after training pre-trained model with CT task (CT baseline in this case). The affinity score for the intermediate fine-tuned model is -0.763, while the pre-trained model has an affinity score of -3.471. It was observed that the affinity score for the intermediate fine-tuned model is much larger than that of the pre-trained model. This is equivalent to say that with CT, the model is further away from the baseline model compared to the pre-trained model. This result suggests that the training on CT has a large negative impact on the performance of the subsequent CR task. This matches with the negative transfer we observed for the CT$\rightarrow$CR.


\begin{table}[t]
\caption{Task Affinity Analysis Results}
\label{tab:task-affinity}
\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{|l|c|}
\hline
\textbf{Models}   & \textbf{Task Affinity Scores} \\ \hline
CR$\rightarrow$CT & -6.121                        \\ \hline
CT\_Pre-train     & -6.987                        \\ \hline
CT$\rightarrow$CR & -0.763                        \\ \hline
CR\_Pre-train     & -3.471                        \\ \hline
\end{tabular}%
}
\end{table}

% \begin{center}
%     \begin{tabular}{| l | l |}
%     \hline    
%     \multicolumn{2}{|c|}{\textbf{Task Affinity Results}} \\
%     \hline
%     Finetuning Chain            &    Task Affinity Score     \\
%     \hline
%     CR$\rightarrow$CT          &   -6.121      \\
%     \hline
%     CT\_DEFAULT     &   -6.987      \\
%     \hline
%     CT$\rightarrow$CR          &   -0.763      \\
%     \hline
%     CR\_DEFAULT     &   -3.471      \\
%     \hline
%     CD$\rightarrow$DD          &   -0.241      \\
%     \hline
%     DD\_DEFAULT     &   -0.2586     \\
%     \hline
%     \end{tabular}
% \end{center}

\observation{Task affinity can only explain the negative transfer for CT$\rightarrow$CR, but contradicts to the positive transfer we observed for CR$\rightarrow$CT. Thus, task affinity is not a good measurement.}

%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 4: Task affinity can only explain the negative transfer for CT$\rightarrow$CR, but contradicts to the positive transfer we observed for CR$\rightarrow$CT. Thus, task affinity is not a good measurement.} 
%\end{mdframed}

% \hl{we cannot say that it makes sense for one out of 3 and for others it doesn't. Task affinity alone doesn't explain and there must be other factors should be the finding}
% \subsection{Task: Retrieval VS Classification}
% In order to perform an analysis to compare the effect of CD's two task variants, similar code retrieval (retrieval task) and the prediction of semantic equivalence for a pair of code (classification task), on DD's performance (classification task), we present the results of the performances of fine-tuning chain models CD$\rightarrow$DD and DD$\rightarrow$CD in Table \ref{tab:cd-dd-type}. For illustration purposes, we use \textit{classification CD} and \textit{retrieval CD} to refer to the two task variants of CD. \hl{don't see any such thing on mentioned table 4}

% We used the corresponding variants of datasets (retrieval CD dataset and converted classification CD dataset) to fine-tune CD while keeping the training dataset for DD the same (since DD is a classification task and does not have task variants).

% \noindent\textit{\textbf{Type1 VS Type3:}} Recall that Type1 involves fine-tuning retrieval CD before DD, while Type3 refers to fine-tuning classification CD before DD. Table \ref{tab:cd-dd-type} indicates that, for task ordering CD$\rightarrow$DD, changing from retrieval CD to classification CD enhances the performance of DD for most of the fine-tuning chain models. 

% In addition, the CD BCB dataset in CodeXGLUE is another classification CD dataset that researchers have widely used to evaluate their classification CD models. Therefore, we compare the model performances after training with the converted classification CD dataset with that of BCB dataset, and find that the model performance after training with the converted classification CD dataset (0.6556 in F-1 score) is much lower than that of the BCB dataset (0.941 in F-1 score). We attribute this performance gap to the following possible reasons:

% (1) Our converted dataset contains different programs than the BCB dataset as we built our converted dataset from the CD\_POJ104 dataset.

% (2) The BCB dataset is much larger than our dataset. Our dataset comprises 64000 data samples, where half of the samples are positive samples and the other half are negative. In contrast, BCB dataset consists of 901028 data samples with an equal ratio of positive and negative examples. 



% \begin{mdframed}[roundcorner=10pt]
% \textbf{Finding 7:  Task type similarity may be a factor that helps explain Pattern 2.} 
% \end{mdframed}

% \hl{rewrite this finding. it's not able explain pattern 2. Also you shouldn't referr to a pattern in finding. elaborate the finding}

% \begin{table}[ht]
% \caption{Classification CD and Retrieval CD's effect on DD}
% \label{tab:cd-dd-type}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l d|l|}
% \hline
% \textbf{Task Ordering}                     & \textbf{Type1 Performance} & \textbf{Type3 Performance} \\ \hline
% CR$\rightarrow$CD$\rightarrow$DD                & 0.610                      & 0.62295                    \\ \hline
% CD$\rightarrow$DD                               & 0.619                      & 0.6197                     \\ \hline
% CD$\rightarrow$CR$\rightarrow$DD                & 0.626                      & 0.6255                     \\ \hline
% CT$\rightarrow$CD$\rightarrow$DD                & 0.610                      & 0.6260                     \\ \hline
% CD$\rightarrow$CT$\rightarrow$DD                & 0.628                      & 0.62188                    \\ \hline
% CT$\rightarrow$CR$\rightarrow$CD$\rightarrow$DD & 0.605                      & 0.6274                     \\ \hline
% CT$\rightarrow$CD$\rightarrow$CR$\rightarrow$DD & 0.614                      & 0.61969                    \\ \hline
% CR$\rightarrow$CT$\rightarrow$CD$\rightarrow$DD & 0.607                      & 0.6292                     \\ \hline
% CR$\rightarrow$CD$\rightarrow$CT$\rightarrow$DD & 0.619                      & 0.63103                    \\ \hline
% CD$\rightarrow$CT$\rightarrow$CR$\rightarrow$DD & 0.606                      & 0.6383                     \\ \hline
% CD$\rightarrow$CR$\rightarrow$CT$\rightarrow$DD & 0.615                      & 0.62811                    \\ \hline
% \end{tabular}%
% }
% \end{table}


% \begin{center}
%     \begin{tabular}{|l | l | l|}
%     \hline
%     \multicolumn{3}{|c|}{\textbf{Type1 VS Type3}} \\
%     \hline
%     Finetuning Chain      &       Type1 Performance   &   Type3 Performance\\
%     \hline
%     CR$\rightarrow$CD$\rightarrow$DD      &       0.610                &      0.62295\\
%     \hline
%     CD$\rightarrow$DD          &       0.619                &      0.6197\\
%     \hline
%     CD$\rightarrow$CR$\rightarrow$DD      &       0.626                &      0.6255\\
%     \hline
%     CT$\rightarrow$CD$\rightarrow$DD      &       0.610                &      0.6260\\
%     \hline
%     CD$\rightarrow$CT$\rightarrow$DD      &       0.628                &      0.62188\\
%     \hline
%     CT$\rightarrow$CR$\rightarrow$CD$\rightarrow$DD  &       0.605                &      0.6274\\
%     \hline
%     CT$\rightarrow$CD$\rightarrow$CR$\rightarrow$DD  &       0.614                &      0.61969\\
%     \hline
%     CR$\rightarrow$CT$\rightarrow$CD$\rightarrow$DD  &       0.607                &      0.6292 \\
%     \hline
%     CR$\rightarrow$CD$\rightarrow$CT$\rightarrow$DD  &       0.619                &      0.63103\\
%     \hline
%     CD$\rightarrow$CT$\rightarrow$CR$\rightarrow$DD  &       0.606                &      0.6383\\
%     \hline
%     CD$\rightarrow$CR$\rightarrow$CT$\rightarrow$DD  &       0.615                &      0.62811\\
%     \hline
%     \end{tabular}
% \end{center}


\subsection{Model: Probing Tasks}

We train a logistic regression classifier for every fine-tuning chain model in this study with the probing datasets from \cite{karmakar2021pre}. Due to the space limit, we only present the probing task performances of chains that end with CT (i.e. CT is the target task) along with the fine-tuning chain model performances in Table \ref{tab:probing-ct}. The probing results for other chains are in our replication package~\cite{replication}. Recall that the mean of the classifier accuracies trained on the feature vectors from all 12 layers of the encoder was referred to as the overall probing task performance (Section \ref{sec:modelanalysis}). It is worth noting that our focus is more on the probing task performance difference between models instead of raw performance value for each model~\cite{karmakar2021pre}. Then, we conduct Spearman correlation between probing task and target task performances for every target task across different fine-tuning chain models whose task orderings end with this target task. The correlation coefficients are shown in Table \ref{tab:probingvstarget}. 

Since the performance of probing tasks can be treated as an indicator of the acquisition of particular language skills, we provide possible explanations for the task ordering patterns we found (Section \ref{sec:results}) below:

\textit{Explanation for \textbf{Pattern 2: }}The performances of fine-tuning chain models whose task orderings end with CR have a higher correlation with TYP’s performance (correlation coefficient 0.638) than those of fine-tuning chain models whose task orderings end with CT (correlation coefficient 0.342). This suggests that, for CR to perform better, the model tends to pay more attention to code semantic information when it is fine-tuned than CT does. This can also be seen from the baseline performance where TYP’s performance of CR baseline is higher than that of CT, which indicates CR learns code semantic information better than CT. Also, TYP’s performance trained on the vectors from CR baseline (90) is higher than that of fine-tuning chain model CT$\rightarrow$CR (87.833). We posit that the reason why CT$\rightarrow$CR is a negative transfer task ordering pattern is because CT doesn’t care about TYP as much as CR, so it might have hurt the subsequent CR’s effectiveness of learning code semantic information, which causes CT$\rightarrow$CR to perform worse than CR.

% \textit{Explanation for \textbf{Pattern 2: }}CD$\rightarrow$DD is anther negative transfer pattern. Similar to CT$\rightarrow$CR, we found fine-tuning chain models whose task orderings end with DD do pay more attention to both syntactic (correlation coefficient 0.660) and semantic information (correlation coefficient 0.556) than chain models whose task orderings end with CD do. In addition, CD baseline has lower probing task performances for both AST and TYP than DD. We believe the reason for this negative transfer could be that CD negatively impacts DD's learning of both syntactic and semantic information, which leads to a performance degradation of DD.

However, probing task performance and its correlation with target task performance can not provide enough evidence to explain why \textbf{Pattern 1} is a positive transfer pattern. It's possible that other factors such as dataset size may play a role in explaining it.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Correlation between Probing Task Performances and Target Task Performances}
\label{tab:probingvstarget}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|cccc|cccl|}
\hline
\textbf{} & \multicolumn{4}{c|}{\textbf{AST}} & \multicolumn{4}{c|}{TYP} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Correlation\\ Coefficients\end{tabular}} & CD & DD & CR & CT & CD & DD & CR & CT \\ \cline{2-9} 
 & 0.223 & 0.660 & 0.158 & 0.069 & 0.151 & 0.556 & 0.638 & 0.342 \\ \hline
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\caption{Probing Task Performances and Model Performances (CT)}
\label{tab:probing-ct}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Chain Models} & \textbf{\begin{tabular}[c]{@{}c@{}}AST Mean \\ Accuracies\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TYP Mean \\ Accuracies\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Model Perfor-\\ -mance (BLEU)\end{tabular}} \\ \hline
CT & 77.792 & 88.500 & 70.881 \\ \hline
CR$\rightarrow$CT & 79.000 & 88.750 & 74.242 \\ \hline
CD$\rightarrow$CT & 78.958 & 87.708 & 70.879 \\ \hline
DD$\rightarrow$CT & 79.042 & 88.667 & 70.839 \\ \hline
CD$\rightarrow$CR$\rightarrow$CT & 78.875 & 88.042 & 75.058 \\ \hline
CD$\rightarrow$DD$\rightarrow$CT & 78.833 & 88.750 & 71.000 \\ \hline
CR$\rightarrow$CD$\rightarrow$CT & 77.792 & 85.708 & 73.957 \\ \hline
CR$\rightarrow$DD$\rightarrow$CT & 79.250 & 86.083 & 74.118 \\ \hline
DD$\rightarrow$CD$\rightarrow$CT & 78.708 & 87.500 & 70.739 \\ \hline
DD$\rightarrow$CR$\rightarrow$CT & 78.208 & 83.833 & 74.113 \\ \hline
CD$\rightarrow$CR$\rightarrow$DD$\rightarrow$CT & 77.083 & 86.167 & 74.204 \\ \hline
CD$\rightarrow$DD$\rightarrow$CR$\rightarrow$CT & 80.125 & 83.917 & 74.606 \\ \hline
CR$\rightarrow$CD$\rightarrow$DD$\rightarrow$CT & 79.667 & 86.750 & 73.882 \\ \hline
CR$\rightarrow$DD$\rightarrow$CD$\rightarrow$CT & 78.792 & 83.083 & 74.145 \\ \hline
DD$\rightarrow$CD$\rightarrow$CR$\rightarrow$CT & 79.792 & 83.167 & 73.950 \\ \hline
DD$\rightarrow$CR$\rightarrow$CD$\rightarrow$CT & 79.667 & 86.667 & 73.942 \\ \hline
\end{tabular}%
}
\end{table}

\observation{Intermediate tasks' learning effectiveness of code syntactic or semantic skills may have an impact on the learning of the target task and its performance. However, other factors may also play a role.}
%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 5:  Intermediate tasks' learning effectiveness of code syntactic or semantic skills may have an impact on the learning of the target task and its performance. However, other factors may also play a role.} 
%\end{mdframed}


\subsection{Model: Attention Analysis} 
%\hl{without the result what am I supposed to look at!}
We present the results of our attention analysis for syntax tokens and abstract syntax tree structures in Figures \ref{fig:attention_syntax} and \ref{fig:attention_ast}, respectively. The X-axis represents the layer numbers and the Y-axis represents the attention scores. The curves in the figures indicate the average attention scores of a model across 12 layers. We observed that for the CR$\rightarrow$CT fine-tuning chain model, the average attention scores were higher than those of the CT baseline model in both syntax tokens and abstract syntax tree structure. This is consistent with the positive transfer (\textbf{Pattern 1}) we observed for CR$\rightarrow$CT task ordering. Conversely, for the CT$\rightarrow$CR fine-tuning chain model (lower sub-graphs), the average attention scores were lower than those of the CR baseline model for all cases in both syntax tokens and abstract syntax tree structure, which matches with the negative transfer (\textbf{Pattern 2}) we observed for CT$\rightarrow$CR. Based on our analysis, we can conclude that the performance of a model is positively correlated with the attention scores it receives across all 12 layers for both abstract syntax structure and syntax tokens. %In other words, a model that exhibits higher attention scores across these layers is likely to perform better, while a model with lower attention scores across the same layers is likely to perform worse.



% On one hand, the average attention scores for both abstract syntax tree structure and syntax tokens of CR$\rightarrow$CT fine-tuning chain model are higher than CT baseline, where CR boosts CT's performance (\textbf{Pattern 3}). On the other hand, we observed that the baseline CR model has higher average attention values than CT$\rightarrow$CR fine-tuning chain model where fine-tuning CT before harms CR's performance (\textbf{Pattern 1}). Based on these observations, we conclude that the task orderings that lead to a positive transfer would have higher average attention scores for both abstract syntax tree structure and syntax tokens than those of baseline models. However, for \textbf{Pattern 2}, we did not observe significant difference in the average attention values between CD$\rightarrow$DD model and the DD baseline. Specifically, the average attention values for both the CD$\rightarrow$DD model and the DD baseline model are close.

%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 6: the average attention scores of the model for both abstract syntax tree structure and syntax tokens can be a factor that explains the positive and negative transfers of knowledge.} 
%\end{mdframed}

\observation{Average attention scores of the model for both abstract syntax tree structure and syntax tokens can be a factor that explains the positive and negative transfers of knowledge.}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/syntax_diff.png}
    \caption{Attention weight experimental results on syntax tokens}
    \label{fig:attention_syntax}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/ast_diff.png}
    \caption{Attention weight experimental results on abstract syntax tree elements}
    \label{fig:attention_ast}
\end{figure*}


\subsection{Time Cost Effective Analysis}
\label{sec:costeffect}
%\hl{which column is relative transfer gains?}
%\hl{Move this to implications}
To determine the most efficient fine-tuning approaches for improving target task performance, we gathered performance gains measured by relative performance gain~\cite{vu2020exploring} (Section \ref{sec:timeanalysis}), training time (in hours), time difference between fine-tuning chain models and baseline models (Section \ref{sec:timeanalysis}), and effective ratio (Section \ref{sec:timeanalysis}) for all fine-tuning chain models that demonstrated positive transfer for target tasks. We found that the values for relative performance gain and effective ratio were too small to be easily discerned, so we multiplied them by 100 to facilitate visualization. For this analysis, we set the effective ratio threshold value at 1.697, which is the mean of all effective ratios. We consider fine-tuning chain models with an effective ratio below the threshold to be non-cost-effective. Based on our analysis, we identified seven task orderings as non-cost-effective, while the four remaining task orderings (CR$\rightarrow$CT, CD$\rightarrow$CR$\rightarrow$CT, DD$\rightarrow$CR$\rightarrow$CT, and CR$\rightarrow$DD$\rightarrow$CT) were deemed cost-effective. We recommend choosing the task orderings with effective ratios higher than the threshold value as they bring positive transfer and are cost-effective. We use mean for calculating threshold in our analysis, but it can be replaced by other standard metrics, such as median or a metric defined by the users. 

%\begin{mdframed}[roundcorner=10pt]
%\textbf{Finding 7: Using intermediate SE tasks may be beneficial for improving model performance, but it's crucial to consider the trade-offs between training time and performance gains. It's important to note that the task ordering with the maximum performance improvement may not always be the optimal choice.} 
%\end{mdframed}

\observation{Using intermediate SE tasks may be beneficial for improving model performance, but it's crucial to consider the trade-offs between training time and performance gains. Task ordering with the maximum performance improvement may not always be the optimal choice.}

\begin{table}[t]
\caption{Performance Gain and the Corresponding Training Time}
\label{tab:time-improv}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Fine-tuning Chain Models} & \textbf{\begin{tabular}[c]{@{}c@{}}\textbf{Relative Perfor-}\\ \textbf{-mance Gain(\%)}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Time\\ (Hour)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\bm{\mathit{\Delta}}$Time \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Effective \\ Ratio(\%)\end{tabular}} \\ \hline
CT & / & 4 & 0 & / \\ \hline
CR$\rightarrow$CT & 4.742 & 6 & 2 & 2.371 \\ \hline
CR$\rightarrow$CD$\rightarrow$CT & 4.340 & 6.633 & 2.633 & 1.648 \\ \hline
CD$\rightarrow$CR$\rightarrow$CT & 5.893 & 6.633 & 2.633 & 2.238 \\ \hline
DD$\rightarrow$CR$\rightarrow$CT & 4.560 & 6.500 & 2.500 & 1.824 \\ \hline
CR$\rightarrow$DD$\rightarrow$CT & 4.567 & 6.500 & 2.500 & 1.827 \\ \hline
DD$\rightarrow$CR$\rightarrow$CD$\rightarrow$CT & 4.319 & 7.133 & 3.133 & 1.379 \\ \hline
DD$\rightarrow$CD$\rightarrow$CR$\rightarrow$CT & 4.330 & 7.133 & 3.133 & 1.382 \\ \hline
CR$\rightarrow$DD$\rightarrow$CD$\rightarrow$CT & 4.605 & 7.133 & 3.133 & 1.470 \\ \hline
CR$\rightarrow$CD$\rightarrow$DD$\rightarrow$CT & 4.234 & 7.133 & 3.133 & 1.351 \\ \hline
CD$\rightarrow$DD$\rightarrow$CR$\rightarrow$CT & 5.255 & 7.133 & 3.133 & 1.677 \\ \hline
CD$\rightarrow$CR$\rightarrow$DD$\rightarrow$CT & 4.688 & 7.133 & 3.133 & 1.496 \\ \hline
\end{tabular}%
}
\end{table}



% \begin{table}[ht]
% \caption{Performance Gain and the Corresponding Training Time}
% \label{tab:time-improv}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \textbf{Task Orderings}                     & \textbf{Performance Gain(\%)} & \textbf{Time(Hour)} & \textbf{$\bm{\mathit{\Delta}}$ Time}    & \textbf{Effective Ratio} \\ \hline
% CD                                              & /                  & 0.6333   &0                   & /                        \\ \hline
% CT$\rightarrow$CD                               & 0.2301             & 4.6333   &4                   & 0.05753                  \\ \hline
% CR                                              & /                  & 2        &0                   & /                        \\ \hline
% CD$\rightarrow$CR                               & 0.0968             & 2.6333   &0.6333              & 0.15285                  \\ \hline
% DD$\rightarrow$CR                               & 0.1835             & 2.5      &0.5                 & 0.36700                  \\ \hline
% DD$\rightarrow$CD$\rightarrow$CR                & 0.3255             & 3.1333   &1.1333              & 0.28721                  \\ \hline
% CD$\rightarrow$DD$\rightarrow$CR                & 0.0628             & 3.1333   &1.1333              & 0.05541                  \\ \hline
% CT                                              & /                  & 4        &0                   & /                        \\ \hline
% CR$\rightarrow$CT                               & 4.7418             & 6        &2                   & 2.37090                  \\ \hline
% CR$\rightarrow$CD$\rightarrow$CT                & 4.3397             & 6.6333   &2.6333              & 1.64801                  \\ \hline
% CD$\rightarrow$CR$\rightarrow$CT                & 5.893              & 6.6333   &2.6333              & 2.23788                  \\ \hline
% CD$\rightarrow$DD$\rightarrow$CT                & 0.1679             & 5.1333   &1.1333              & 0.14815                  \\ \hline
% DD$\rightarrow$CR$\rightarrow$CT                & 4.5598             & 6.5      &2.5                 & 1.82392                  \\ \hline
% CR$\rightarrow$DD$\rightarrow$CT                & 4.5668             & 6.5      &2.5                 & 1.82672                  \\ \hline
% DD$\rightarrow$CR$\rightarrow$CD$\rightarrow$CT & 4.3185             & 7.1333   &3.1333              & 1.37826                  \\ \hline
% DD$\rightarrow$CD$\rightarrow$CR$\rightarrow$CT & 4.3298             & 7.1333   &3.1333              & 1.38187                  \\ \hline
% CR$\rightarrow$DD$\rightarrow$CD$\rightarrow$CT & 4.6049             & 7.1333   &3.1333              & 1.46966                  \\ \hline
% CR$\rightarrow$CD$\rightarrow$DD$\rightarrow$CT & 4.2339             & 7.1333   &3.1333              & 1.35126                 \\ \hline
% CD$\rightarrow$DD$\rightarrow$CR$\rightarrow$CT & 5.2553             & 7.1333   &3.1333              & 1.67724                 \\ \hline
% CD$\rightarrow$CR$\rightarrow$DD$\rightarrow$CT & 4.6881             & 7.1333   &3.1333              & 1.49622                 \\ \hline
% \end{tabular}%
% }
% \end{table}

% \begin{center}
%     \begin{tabular}{|l | l | l| l |}
%     \hline
%     \multicolumn{4}{|c|}{\textbf{Performance Improvement Time Records}} \\
%     \hline
%     Finetuning Chain                                              &       Delta(\%)         &      Time(Hour)     &   Effective Ratio\\
%     \hline      
%     CD                                                      &       /                   &      0.6333       &   /       \\
%     \hline
%     CT$\rightarrow$CD                                       &       0.2301              &      4.6333       &   0.04966\\
%     \hline
%     CR                                                      &       /                   &      2            &   /       \\
%     \hline
%     CD$\rightarrow$CR                                       &       0.0968              &      2.6333       &   0.03676\\
%     \hline
%     DD$\rightarrow$CR                                       &       0.1835              &      2.5          &   0.07340\\
%     \hline
%     DD$\rightarrow$CD$\rightarrow$CR                        &       0.3255              &      3.1333       &   0.10388\\
%     \hline
%     CD$\rightarrow$DD$\rightarrow$CR                        &       0.0628              &      3.1333       &   0.02004\\
%     \hline
%     CT                                                      &       /                   &      4            &   /       \\
%     \hline
%     CR$\rightarrow$CT                                       &       4.7418              &      6            &   0.79030\\
%     \hline
%     CR$\rightarrow$CD$\rightarrow$CT                        &       4.3397              &      6.6333       &   0.65423\\
%     \hline
%     CD$\rightarrow$CR$\rightarrow$CT                        &       5.893               &      6.6333       &   0.88840\\
%     \hline
%     CD$\rightarrow$DD$\rightarrow$CT                        &       0.1679              &      5.1333       &   0.03271\\
%     \hline
%     DD$\rightarrow$CR$\rightarrow$CT                        &       4.5598              &      6.5          &   0.70151\\
%     \hline
%     CR$\rightarrow$DD$\rightarrow$CT                        &       4.5668              &      6.5          &   0.70258\\
%     \hline
%     DD$\rightarrow$CR$\rightarrow$CD$\rightarrow$CT         &       4.3185              &      7.1333       &   0.60540\\
%     \hline
%     DD$\rightarrow$CD$\rightarrow$CR$\rightarrow$CT         &       4.3298              &      7.1333       &   0.60698\\
%     \hline
%     CR$\rightarrow$DD$\rightarrow$CD$\rightarrow$CT         &       4.6049              &      7.1333       &   0.64555\\
%     \hline
%     CR$\rightarrow$CD$\rightarrow$DD$\rightarrow$CT         &       4.2339              &      7.1333       &   0.59354\\
%     \hline
%     CD$\rightarrow$DD$\rightarrow$CR$\rightarrow$CT         &       5.2553              &      7.1333       &   0.73673\\
%     \hline
%     CD$\rightarrow$CR$\rightarrow$DD$\rightarrow$CT         &       4.6881              &      7.1333       &   0.65721\\
%     \hline
%     \end{tabular}
% \end{center}

==> figures/06-implications.tex <==
\section{Implications}
\label{sec:impl}
Based on our findings, we provide the following implications for researchers and software practitioners.

\textit{\textbf{Implications for researchers:}} First, our findings in RQ1 demonstrated that some tasks' performances can either get boosted or hurt depending on the fine-tuning ordering of all tasks, while the performance may always drop for some other tasks no matter what intermediate tasks are fine-tuned before them. We believe a study on a more extensive group of SE tasks is needed to uncover more patterns and opportunities to further improve the performances of certain tasks. Second, to answer RQ2 from the perspective of task similarity, we took task affinity (Section \ref{sec:SE task sim}) as a measure in this study. However, this measure does not sufficiently explain the two task ordering patterns we identified in Section \ref{sec:results}. This might be happening due to the inability of the task affinity metric to capture task similarity. Hence, researchers should look into designing metrics to measure SE task similarity, which can efficiently reflect the transferability between SE tasks. Finally, we picked the mean effective ratio across all positive transfer fine-tuning chain models as the threshold to determine whether it's cost-effective to improve the target task performance (Section \ref{sec:costeffect}). A promising future direction would be to build a machine learning model that can automatically predict a reasonable threshold and then recommend the proper task orderings that can best improve the target task performance.

\textit{\textbf{Implications for practitioners:}} It may be intuitive to believe that the target task whose training data has a small number of data samples would always benefit from a preceding fine-tuned intermediate task with more training data, and the intermediate task with a large amount of training data may always lead to a positive transfer to downstream tasks. However, our findings suggest that this is not always the case. In order to improve task performance, we recommend practitioners to consider syntactic and semantic similarities between task training datasets when performing intermediate task fine-tuning rather than blindly trying to collect more training data. In addition, to make the model-building process more cost-efficient with intermediate task fine-tuning, practitioners can set their own effective ratio thresholds to select intermediate tasks to improve target task performance based on their resource budget.  

==> figures/07-threats.tex <==
\section{Threats To Validity}
\label{sec:ttv}
We have taken all reasonable steps to mitigate potential threats that could hamper the validity of this study, it is still possible that our mitigation strategies might not have been effective.

\textbf{Construct validity:} We used the evaluation metrics in CodeX-\\GLUE to assess the performance of fine-tuning chain models. If other metrics are used, the performance gain could differ. However, our goal was not to identify an absolute gain through tbut to highlight the possibility of performance gain, hence this threat does not impact the validity of our findings.
%Our model evaluation results may change depending on the metrics used. It is necessary to extend the model evaluations by using a variety of state-of-the-art metrics. We leave the evaluations with other metrics to our future work.

\textbf{Internal validity:} In this study, our probing setup does not cover all possible aspects of source code. However, to make our experiments manageable, we focused on exploring semantic and syntactic code properties learned by a model. Then, we only took two probing tasks (AST and TYP) from~\cite{karmakar2021pre} to estimate the learning effectiveness of code syntactic and semantic information by a fine-tuned model. Other variants of these two probing tasks may better estimate the model's acquisition of syntactic and semantic information. Finally, the linear classifier used for probing might be limited in its ability to learn more complex encoding of code properties. However, it was used in many probing approaches~\cite{karmakar2021pre, troshin2022probing}, demonstrating promising and reliable results.

%Similarly, our approaches for measuring the syntactic and semantic similarity between datasets might have their own limitations, which might have missed some aspects of data similarity that could be considered influential on SE task transferability. For attention analysis, our results may not apply to the syntax tokens and abstract syntax structures other than the ones we analyzed in this study.% do we question their approaches from the NLP papers? 

%To identify fine-tuning chain models of positive and negative transfer, we only focused on those whose performances show statistically significant differences (across 10-fold cross validation) from the corresponding baseline models. Other task ordering patterns may emerge when considering models with no statistically significant differences. 

\textbf{External validity:} Our findings may not be generalizable to all pre-trained language models of source code. Since the programming languages involved in our fine-tuning process are only Java, C/C++, and C\#, our findings may not apply to models fine-tuned with other programming languages. Moreover, we conducted our experiments on only four SE tasks, and we analyzed two task ordering patterns from them. It is possible that the conclusions from these analyses may not apply to other SE tasks, and their task orderings. 

==> figures/08-conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

We conducted the first empirical study on the impact of fine-tuning SE task orderings on target task performance. We argue that the results of our fine-tuning chain model evaluations and associated discussions can provide SE researchers and practitioners with a deeper understanding about the transferability between various SE tasks, as well as the training time and performance gain trade-off when selecting task orderings for a given target task to maximize its performance.

Our study sheds light on relevant factors that may be helpful in explaining the reasons why certain task orderings (task ordering patterns) can always bring performance gain/loss to target tasks. We believe that more factors and measures should be considered to explain those patterns, and an exploration on a more extensive group of SE tasks and more pre-trained language models should be performed to further understand this impact. %We leave these as our future works. 
